Benchmarking System One decision models against trained classifiers and language models for automated decision gates

Software that hands branching decisions to a model needs a declared option and a probability it can threshold. Typed decision models, also called System One models, return such probabilities without generating text, while supervised classifiers and generative language models are the established alternatives. One harness sends eight decision-model checkpoints from six families, including the hosted model Jev, and four open generative models from three developers the same semantic requests, and scores trained and zero-shot classifiers on the same workflow, intent, emotion and social-science items. With task labels, a fine-tuned DeBERTa-v3-large has the highest observed accuracy on every labeled benchmark but one. Without labels, no decision model is significantly more accurate than Jev on workflows or intents, but Gemma-4-31B matches it on workflows and exceeds it on CLINC-150 at higher cost and latency. Stated probabilities of generative models become unreadable when replies miss the key format, whereas key likelihoods avoid this but can saturate. A guaranteed 5 percent risk leaves Jev 0.528 of the intent decisions, and an in-scope threshold still accepts 0.310 of out-of-scope requests. On typed-decisions, swapping yes and no flips 50.5 answers per hundred for Jev and at least 16.8 for every generative model tested, against at most 6.5 for four fine-tuned decision checkpoints. Exposure to a benchmark's training data explains the largest lead of an open checkpoint, which vanishes on rater-labeled emotions. An intent-trained first stage escalating to Gemma-4-31B reaches that model's accuracy at about Jev's price. The results yield condition-dependent design rules for automated decision gates.

==> tables/t06_names.tex <==
% Generated by shared/src/t01_tables.py. Do not edit by hand.
% Every numeric cell is a num-macro from numbers.tex; -- means that
% model has no result for this cell yet. Needs paper4a_tables.sty.
\tablestyle
\begin{tabular}{P{0.2850}P{0.1650}N{0.1100}N{0.1100}N{0.1100}N{0.1100}N{0.1100}}
\toprule
\headrow \hdtop{} & \hdtop{} & \hdgroup{three}{Flips per hundred decisions} & \hdtop{} & \hdtop{} \\
\bandrules{3-5}
\headrow \hdsub{Model} & \hdsub{Binary set} & \hdsub{\flipcell{}{Digits}} & \hdsub{\flipcell{}{Random}} & \hdsub{\flipcell{}{Swapped}} & \hdsub{AUC} & \hdsub{Floor} \\
\midrule
\tabhead
\groupspan{seven}{Hosted}
\msw{jev}Jev 1.13.0 & Typed-decisions & \flipcell{\symhalf}{\num{e2.jev.done.k01.flips}} & \flipcell{\symnone}{\num{e2.jev.done.krand.flips}} & \flipcell{\symfull}{\num{e2.jev.done.kswap.flips}} & \num{e2.jev.done.kny.auc} & \num{e2.jev.done.floor} \\
 & Derailment & \flipcell{\symnone}{\num{e2.jev.toxicity.k01.flips}} & \flipcell{\symnone}{\num{e2.jev.toxicity.krand.flips}} & \flipcell{\symfull}{\num{e2.jev.toxicity.kswap.flips}} & \best{\num{e2.jev.toxicity.kny.auc}} & \num{e2.jev.toxicity.floor} \\
 & Power & \flipcell{\symhalf}{\num{e2.jev.power.k01.flips}} & \flipcell{\symhalf}{\num{e2.jev.power.krand.flips}} & \flipcell{\symfull}{\num{e2.jev.power.kswap.flips}} & \num{e2.jev.power.kny.auc} & \num{e2.jev.power.floor} \\
\groupspan{seven}{Open, encoder head}
\msw{layaen}Laya (English) & Typed-decisions & \flipcell{\symfull}{\num{e2.layaen.done.k01.flips}} & \flipcell{\symfull}{\num{e2.layaen.done.krand.flips}} & \flipcell{\symfull}{\num{e2.layaen.done.kswap.flips}} & \num{e2.layaen.done.kny.auc} & \num{e2.layaen.done.floor} \\
 & Derailment & \flipcell{\symfull}{\num{e2.layaen.toxicity.k01.flips}} & \flipcell{\symfull}{\num{e2.layaen.toxicity.krand.flips}} & \flipcell{\symfull}{\num{e2.layaen.toxicity.kswap.flips}} & \num{e2.layaen.toxicity.kny.auc} & \num{e2.layaen.toxicity.floor} \\
 & Power & \flipcell{\symfull}{\num{e2.layaen.power.k01.flips}} & \flipcell{\symfull}{\num{e2.layaen.power.krand.flips}} & \flipcell{\symfull}{\num{e2.layaen.power.kswap.flips}} & \num{e2.layaen.power.kny.auc} & \num{e2.layaen.power.floor} \\
\addlinespace[2.5pt]
\msw{layaml}Laya (multilingual) & Typed-decisions & \flipcell{\symfull}{\num{e2.layaml.done.k01.flips}} & \flipcell{\symfull}{\num{e2.layaml.done.krand.flips}} & \flipcell{\symfull}{\num{e2.layaml.done.kswap.flips}} & \num{e2.layaml.done.kny.auc} & \num{e2.layaml.done.floor} \\
 & Derailment & \flipcell{\symfull}{\num{e2.layaml.toxicity.k01.flips}} & \flipcell{\symfull}{\num{e2.layaml.toxicity.krand.flips}} & \flipcell{\symfull}{\num{e2.layaml.toxicity.kswap.flips}} & \num{e2.layaml.toxicity.kny.auc} & \num{e2.layaml.toxicity.floor} \\
 & Power & \flipcell{\symfull}{\num{e2.layaml.power.k01.flips}} & \flipcell{\symfull}{\num{e2.layaml.power.krand.flips}} & \flipcell{\symfull}{\num{e2.layaml.power.kswap.flips}} & \num{e2.layaml.power.kny.auc} & \num{e2.layaml.power.floor} \\
\groupspan{seven}{Open, decoder head}
\msw{kevsmall}Kev-0.8B & Typed-decisions & \flipcell{\symhalf}{\num{e2.kevsmall.done.k01.flips}} & \flipcell{\symfull}{\num{e2.kevsmall.done.krand.flips}} & \flipcell{\symfull}{\num{e2.kevsmall.done.kswap.flips}} & \num{e2.kevsmall.done.kny.auc} & \num{e2.kevsmall.done.floor} \\
 & Derailment & \flipcell{\symnone}{\num{e2.kevsmall.toxicity.k01.flips}} & \flipcell{\symnone}{\num{e2.kevsmall.toxicity.krand.flips}} & \flipcell{\symhalf}{\num{e2.kevsmall.toxicity.kswap.flips}} & \num{e2.kevsmall.toxicity.kny.auc} & \num{e2.kevsmall.toxicity.floor} \\
 & Power & \flipcell{\symhalf}{\num{e2.kevsmall.power.k01.flips}} & \flipcell{\symhalf}{\num{e2.kevsmall.power.krand.flips}} & \flipcell{\symhalf}{\num{e2.kevsmall.power.kswap.flips}} & \num{e2.kevsmall.power.kny.auc} & \num{e2.kevsmall.power.floor} \\
\addlinespace[2.5pt]
\msw{kevlarge}Kev-9B & Typed-decisions & \flipcell{\symhalf}{\num{e2.kevlarge.done.k01.flips}} & \flipcell{\symhalf}{\num{e2.kevlarge.done.krand.flips}} & \flipcell{\symhalf}{\num{e2.kevlarge.done.kswap.flips}} & \num{e2.kevlarge.done.kny.auc} & \num{e2.kevlarge.done.floor} \\
 & Derailment & \flipcell{\symnone}{\num{e2.kevlarge.toxicity.k01.flips}} & \flipcell{\symnone}{\num{e2.kevlarge.toxicity.krand.flips}} & \flipcell{\symnone}{\num{e2.kevlarge.toxicity.kswap.flips}} & \num{e2.kevlarge.toxicity.kny.auc} & \num{e2.kevlarge.toxicity.floor} \\
 & Power & \flipcell{\symhalf}{\num{e2.kevlarge.power.k01.flips}} & \flipcell{\symhalf}{\num{e2.kevlarge.power.krand.flips}} & \flipcell{\symhalf}{\num{e2.kevlarge.power.kswap.flips}} & \num{e2.kevlarge.power.kny.auc} & \num{e2.kevlarge.power.floor} \\
\addlinespace[2.5pt]
\msw{decider}decider-2b & Typed-decisions & \flipcell{\symhalf}{\num{e2.decider.done.k01.flips}} & \flipcell{\symhalf}{\num{e2.decider.done.krand.flips}} & \flipcell{\symhalf}{\num{e2.decider.done.kswap.flips}} & \num{e2.decider.done.kny.auc} & \num{e2.decider.done.floor} \\
 & Derailment & \flipcell{\symnone}{\num{e2.decider.toxicity.k01.flips}} & \flipcell{\symnone}{\num{e2.decider.toxicity.krand.flips}} & \flipcell{\symhalf}{\num{e2.decider.toxicity.kswap.flips}} & \num{e2.decider.toxicity.kny.auc} & \num{e2.decider.toxicity.floor} \\
 & Power & \flipcell{\symhalf}{\num{e2.decider.power.k01.flips}} & \flipcell{\symhalf}{\num{e2.decider.power.krand.flips}} & \flipcell{\symhalf}{\num{e2.decider.power.kswap.flips}} & \num{e2.decider.power.kny.auc} & \num{e2.decider.power.floor} \\
\addlinespace[2.5pt]
\msw{thisthat}this-that-model-1.0 & Typed-decisions & \flipcell{\symhalf}{\num{e2.thisthat.done.k01.flips}} & \flipcell{\symhalf}{\num{e2.thisthat.done.krand.flips}} & \flipcell{\symhalf}{\num{e2.thisthat.done.kswap.flips}} & \num{e2.thisthat.done.kny.auc} & \num{e2.thisthat.done.floor} \\
 & Derailment & \flipcell{\symnone}{\num{e2.thisthat.toxicity.k01.flips}} & \flipcell{\symnone}{\num{e2.thisthat.toxicity.krand.flips}} & \flipcell{\symnone}{\num{e2.thisthat.toxicity.kswap.flips}} & \num{e2.thisthat.toxicity.kny.auc} & \num{e2.thisthat.toxicity.floor} \\
 & Power & \flipcell{\symhalf}{\num{e2.thisthat.power.k01.flips}} & \flipcell{\symhalf}{\num{e2.thisthat.power.krand.flips}} & \flipcell{\symhalf}{\num{e2.thisthat.power.kswap.flips}} & \num{e2.thisthat.power.kny.auc} & \num{e2.thisthat.power.floor} \\
\addlinespace[2.5pt]
\msw{nimble}Nimble-9B & Typed-decisions & \flipcell{\symhalf}{\num{e2.nimble.done.k01.flips}} & \flipcell{\symhalf}{\num{e2.nimble.done.krand.flips}} & \flipcell{\symhalf}{\num{e2.nimble.done.kswap.flips}} & \num{e2.nimble.done.kny.auc} & \num{e2.nimble.done.floor} \\
 & Derailment & \flipcell{\symhalf}{\num{e2.nimble.toxicity.k01.flips}} & \flipcell{\symhalf}{\num{e2.nimble.toxicity.krand.flips}} & \flipcell{\symhalf}{\num{e2.nimble.toxicity.kswap.flips}} & \num{e2.nimble.toxicity.kny.auc} & \num{e2.nimble.toxicity.floor} \\
 & Power & \flipcell{\symhalf}{\num{e2.nimble.power.k01.flips}} & \flipcell{\symhalf}{\num{e2.nimble.power.krand.flips}} & \flipcell{\symhalf}{\num{e2.nimble.power.kswap.flips}} & \num{e2.nimble.power.kny.auc} & \num{e2.nimble.power.floor} \\
\groupspan{seven}{Generative comparators}
\msw{comptwo}Qwen3.6-27B, verbal & Typed-decisions & \flipcell{\symhalf}{\num{e2.comptwo.done.k01.flips}} & \flipcell{\symfull}{\num{e2.comptwo.done.krand.flips}} & \flipcell{\symfull}{\num{e2.comptwo.done.kswap.flips}} & \num{e2.comptwo.done.kny.auc} & -- \\
 & Derailment & \flipcell{\symhalf}{\num{e2.comptwo.toxicity.k01.flips}} & \flipcell{\symhalf}{\num{e2.comptwo.toxicity.krand.flips}} & \flipcell{\symfull}{\num{e2.comptwo.toxicity.kswap.flips}} & \num{e2.comptwo.toxicity.kny.auc} & -- \\
 & Power & \flipcell{\symhalf}{\num{e2.comptwo.power.k01.flips}} & \flipcell{\symhalf}{\num{e2.comptwo.power.krand.flips}} & \flipcell{\symfull}{\num{e2.comptwo.power.kswap.flips}} & \num{e2.comptwo.power.kny.auc} & -- \\
\addlinespace[2.5pt]
\msw{comptwoll}Qwen3.6-27B, likelihood & Typed-decisions & \flipcell{\symhalf}{\num{e2.comptwoll.done.k01.flips}} & \flipcell{\symhalf}{\num{e2.comptwoll.done.krand.flips}} & \flipcell{\symfull}{\num{e2.comptwoll.done.kswap.flips}} & \num{e2.comptwoll.done.kny.auc} & -- \\
 & Derailment & \flipcell{\symhalf}{\num{e2.comptwoll.toxicity.k01.flips}} & \flipcell{\symhalf}{\num{e2.comptwoll.toxicity.krand.flips}} & \flipcell{\symfull}{\num{e2.comptwoll.toxicity.kswap.flips}} & \num{e2.comptwoll.toxicity.kny.auc} & -- \\
 & Power & \flipcell{\symhalf}{\num{e2.comptwoll.power.k01.flips}} & \flipcell{\symhalf}{\num{e2.comptwoll.power.krand.flips}} & \flipcell{\symfull}{\num{e2.comptwoll.power.kswap.flips}} & \num{e2.comptwoll.power.kny.auc} & -- \\
\addlinespace[2.5pt]
\msw{compgem}Gemma-4-31B, verbal & Typed-decisions & \flipcell{\symhalf}{\num{e2.compgem.done.k01.flips}} & \flipcell{\symhalf}{\num{e2.compgem.done.krand.flips}} & \flipcell{\symfull}{\num{e2.compgem.done.kswap.flips}} & \num{e2.compgem.done.kny.auc} & -- \\
 & Derailment & \flipcell{\symhalf}{\num{e2.compgem.toxicity.k01.flips}} & \flipcell{\symhalf}{\num{e2.compgem.toxicity.krand.flips}} & \flipcell{\symfull}{\num{e2.compgem.toxicity.kswap.flips}} & \best{\num{e2.compgem.toxicity.kny.auc}} & -- \\
 & Power & \flipcell{\symhalf}{\num{e2.compgem.power.k01.flips}} & \flipcell{\symhalf}{\num{e2.compgem.power.krand.flips}} & \flipcell{\symfull}{\num{e2.compgem.power.kswap.flips}} & \best{\num{e2.compgem.power.kny.auc}} & -- \\
\addlinespace[2.5pt]
\msw{compgemll}Gemma-4-31B, likelihood & Typed-decisions & \flipcell{\symhalf}{\num{e2.compgemll.done.k01.flips}} & \flipcell{\symhalf}{\num{e2.compgemll.done.krand.flips}} & \flipcell{\symfull}{\num{e2.compgemll.done.kswap.flips}} & \best{\num{e2.compgemll.done.kny.auc}} & -- \\
 & Derailment & \flipcell{\symhalf}{\num{e2.compgemll.toxicity.k01.flips}} & \flipcell{\symhalf}{\num{e2.compgemll.toxicity.krand.flips}} & \flipcell{\symfull}{\num{e2.compgemll.toxicity.kswap.flips}} & \num{e2.compgemll.toxicity.kny.auc} & -- \\
 & Power & \flipcell{\symhalf}{\num{e2.compgemll.power.k01.flips}} & \flipcell{\symhalf}{\num{e2.compgemll.power.krand.flips}} & \flipcell{\symfull}{\num{e2.compgemll.power.kswap.flips}} & \num{e2.compgemll.power.kny.auc} & -- \\
\addlinespace[2.5pt]
\msw{compmis}Mistral-Small-24B, verbal & Typed-decisions & \flipcell{\symhalf}{\num{e2.compmis.done.k01.flips}} & \flipcell{\symfull}{\num{e2.compmis.done.krand.flips}} & \flipcell{\symfull}{\num{e2.compmis.done.kswap.flips}} & \num{e2.compmis.done.kny.auc} & -- \\
 & Derailment & \flipcell{\symfull}{\num{e2.compmis.toxicity.k01.flips}} & \flipcell{\symhalf}{\num{e2.compmis.toxicity.krand.flips}} & \flipcell{\symfull}{\num{e2.compmis.toxicity.kswap.flips}} & \num{e2.compmis.toxicity.kny.auc} & -- \\
 & Power & \flipcell{\symhalf}{\num{e2.compmis.power.k01.flips}} & \flipcell{\symhalf}{\num{e2.compmis.power.krand.flips}} & \flipcell{\symfull}{\num{e2.compmis.power.kswap.flips}} & \num{e2.compmis.power.kny.auc} & -- \\
\addlinespace[2.5pt]
\msw{compmisll}Mistral-Small-24B, likelihood & Typed-decisions & \flipcell{\symfull}{\num{e2.compmisll.done.k01.flips}} & \flipcell{\symfull}{\num{e2.compmisll.done.krand.flips}} & \flipcell{\symfull}{\num{e2.compmisll.done.kswap.flips}} & \num{e2.compmisll.done.kny.auc} & -- \\*
 & Derailment & \flipcell{\symhalf}{\num{e2.compmisll.toxicity.k01.flips}} & \flipcell{\symhalf}{\num{e2.compmisll.toxicity.krand.flips}} & \flipcell{\symfull}{\num{e2.compmisll.toxicity.kswap.flips}} & \best{\num{e2.compmisll.toxicity.kny.auc}} & -- \\*
 & Power & \flipcell{\symhalf}{\num{e2.compmisll.power.k01.flips}} & \flipcell{\symhalf}{\num{e2.compmisll.power.krand.flips}} & \flipcell{\symfull}{\num{e2.compmisll.power.kswap.flips}} & \num{e2.compmisll.power.kny.auc} & -- \\*
\bottomrule
\end{tabular}
\tablenote{Digits, Random and Swapped are the option-name conditions, AUC is measured under the aligned identifiers and Floor is the test-retest floor. The glyph grades the flips above the model's floor on that set, \symnone\ below one per hundred, \symhalf\ from one to ten and \symfull\ ten or more. A floor that was not measured counts as zero, as it is for every open model on typed-decisions and for every comparator. Bold marks the highest AUC on each set, with ties bolded.}


==> tables/t09_calib_tasks.tex <==
% Generated by shared/src/t01_tables.py. Do not edit by hand.
% Every numeric cell is a num-macro from numbers.tex; -- means that
% model has no result for this cell yet. Needs paper4a_tables.sty.
\tablestyle
\setlength{\tabcolsep}{2pt}
\begin{tabular}{P{0.1600}N{0.0470}Q{0.0930}N{0.0470}Q{0.0930}N{0.0470}Q{0.0930}N{0.0470}Q{0.0930}N{0.0470}Q{0.0930}N{0.0470}Q{0.0930}}
\toprule
\headrow \hdtop{} & \hdgroup{two}{D1} & \hdgroup{two}{D2} & \hdgroup{two}{Derail.} & \hdgroup{two}{Power} & \hdgroup{two}{Emotion} & \hdgroup{two}{Polite.} \\
\bandrules{2-3,4-5,6-7,8-9,10-11,12-13}
\headrow \hdsub{Model} & \hdsub{Ship.} & \hdsub{Scaled} & \hdsub{Ship.} & \hdsub{Scaled} & \hdsub{Ship.} & \hdsub{Scaled} & \hdsub{Ship.} & \hdsub{Scaled} & \hdsub{Ship.} & \hdsub{Scaled} & \hdsub{Ship.} & \hdsub{Scaled} \\
\midrule
\tabhead
\groupspan{thirteen}{Hosted}
\msw{jev}Jev 1.13.0 & \best{\num{rv.ts.jev.doneneutral.ece}} & \num{rv.ts.jev.doneneutral.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.jev.doneneutral.ecescaledlo}, \num{rv.ts.jev.doneneutral.ecescaledhi}]}} & \num{rv.ts.jev.dtwo.ece} & \num{rv.ts.jev.dtwo.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.jev.dtwo.ecescaledlo}, \num{rv.ts.jev.dtwo.ecescaledhi}]}} & \num{rv.ts.jev.toxicity.ece} & \num{rv.ts.jev.toxicity.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.jev.toxicity.ecescaledlo}, \num{rv.ts.jev.toxicity.ecescaledhi}]}} & \num{rv.ts.jev.power.ece} & \num{rv.ts.jev.power.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.jev.power.ecescaledlo}, \num{rv.ts.jev.power.ecescaledhi}]}} & \num{rv.ts.jev.emotion.ece} & \num{rv.ts.jev.emotion.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.jev.emotion.ecescaledlo}, \num{rv.ts.jev.emotion.ecescaledhi}]}} & \num{rv.ts.jev.politeness.ece} & \num{rv.ts.jev.politeness.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.jev.politeness.ecescaledlo}, \num{rv.ts.jev.politeness.ecescaledhi}]}} \\
\groupspan{thirteen}{Open, encoder head}
\msw{layaen}Laya (English) & \num{rv.ts.layaen.doneneutral.ece} & \num{rv.ts.layaen.doneneutral.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.layaen.doneneutral.ecescaledlo}, \num{rv.ts.layaen.doneneutral.ecescaledhi}]}} & -- & -- & \best{\num{rv.ts.layaen.toxicity.ece}} & \best{\num{rv.ts.layaen.toxicity.ecescaled}}\par{\scriptsize\cellnote{[\num{rv.ts.layaen.toxicity.ecescaledlo}, \num{rv.ts.layaen.toxicity.ecescaledhi}]}} & \best{\num{rv.ts.layaen.power.ece}} & \num{rv.ts.layaen.power.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.layaen.power.ecescaledlo}, \num{rv.ts.layaen.power.ecescaledhi}]}} & \num{rv.ts.layaen.emotion.ece} & \num{rv.ts.layaen.emotion.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.layaen.emotion.ecescaledlo}, \num{rv.ts.layaen.emotion.ecescaledhi}]}} & \num{rv.ts.layaen.politeness.ece} & \num{rv.ts.layaen.politeness.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.layaen.politeness.ecescaledlo}, \num{rv.ts.layaen.politeness.ecescaledhi}]}} \\
\msw{layaml}Laya (multilingual) & \num{rv.ts.layaml.doneneutral.ece} & \num{rv.ts.layaml.doneneutral.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.layaml.doneneutral.ecescaledlo}, \num{rv.ts.layaml.doneneutral.ecescaledhi}]}} & \num{rv.ts.layaml.dtwo.ece} & \num{rv.ts.layaml.dtwo.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.layaml.dtwo.ecescaledlo}, \num{rv.ts.layaml.dtwo.ecescaledhi}]}} & \num{rv.ts.layaml.toxicity.ece} & \num{rv.ts.layaml.toxicity.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.layaml.toxicity.ecescaledlo}, \num{rv.ts.layaml.toxicity.ecescaledhi}]}} & \num{rv.ts.layaml.power.ece} & \num{rv.ts.layaml.power.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.layaml.power.ecescaledlo}, \num{rv.ts.layaml.power.ecescaledhi}]}} & \num{rv.ts.layaml.emotion.ece} & \num{rv.ts.layaml.emotion.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.layaml.emotion.ecescaledlo}, \num{rv.ts.layaml.emotion.ecescaledhi}]}} & \num{rv.ts.layaml.politeness.ece} & \best{\num{rv.ts.layaml.politeness.ecescaled}}\par{\scriptsize\cellnote{[\num{rv.ts.layaml.politeness.ecescaledlo}, \num{rv.ts.layaml.politeness.ecescaledhi}]}} \\
\groupspan{thirteen}{Open, decoder head}
\msw{kevsmall}Kev-0.8B & \num{rv.ts.kevsmall.doneneutral.ece} & \num{rv.ts.kevsmall.doneneutral.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.kevsmall.doneneutral.ecescaledlo}, \num{rv.ts.kevsmall.doneneutral.ecescaledhi}]}} & \num{rv.ts.kevsmall.dtwo.ece} & \num{rv.ts.kevsmall.dtwo.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.kevsmall.dtwo.ecescaledlo}, \num{rv.ts.kevsmall.dtwo.ecescaledhi}]}} & \num{rv.ts.kevsmall.toxicity.ece} & \num{rv.ts.kevsmall.toxicity.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.kevsmall.toxicity.ecescaledlo}, \num{rv.ts.kevsmall.toxicity.ecescaledhi}]}} & \num{rv.ts.kevsmall.power.ece} & \num{rv.ts.kevsmall.power.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.kevsmall.power.ecescaledlo}, \num{rv.ts.kevsmall.power.ecescaledhi}]}} & \num{rv.ts.kevsmall.emotion.ece} & \num{rv.ts.kevsmall.emotion.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.kevsmall.emotion.ecescaledlo}, \num{rv.ts.kevsmall.emotion.ecescaledhi}]}} & \num{rv.ts.kevsmall.politeness.ece} & \num{rv.ts.kevsmall.politeness.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.kevsmall.politeness.ecescaledlo}, \num{rv.ts.kevsmall.politeness.ecescaledhi}]}} \\
\msw{kevlarge}Kev-9B & \num{rv.ts.kevlarge.doneneutral.ece} & \num{rv.ts.kevlarge.doneneutral.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.kevlarge.doneneutral.ecescaledlo}, \num{rv.ts.kevlarge.doneneutral.ecescaledhi}]}} & \num{rv.ts.kevlarge.dtwo.ece} & \num{rv.ts.kevlarge.dtwo.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.kevlarge.dtwo.ecescaledlo}, \num{rv.ts.kevlarge.dtwo.ecescaledhi}]}} & \num{rv.ts.kevlarge.toxicity.ece} & \num{rv.ts.kevlarge.toxicity.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.kevlarge.toxicity.ecescaledlo}, \num{rv.ts.kevlarge.toxicity.ecescaledhi}]}} & \num{rv.ts.kevlarge.power.ece} & \best{\num{rv.ts.kevlarge.power.ecescaled}}\par{\scriptsize\cellnote{[\num{rv.ts.kevlarge.power.ecescaledlo}, \num{rv.ts.kevlarge.power.ecescaledhi}]}} & \num{rv.ts.kevlarge.emotion.ece} & \num{rv.ts.kevlarge.emotion.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.kevlarge.emotion.ecescaledlo}, \num{rv.ts.kevlarge.emotion.ecescaledhi}]}} & \num{rv.ts.kevlarge.politeness.ece} & \num{rv.ts.kevlarge.politeness.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.kevlarge.politeness.ecescaledlo}, \num{rv.ts.kevlarge.politeness.ecescaledhi}]}} \\
\msw{decider}decider-2b & \num{rv.ts.decider.doneneutral.ece} & \num{rv.ts.decider.doneneutral.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.decider.doneneutral.ecescaledlo}, \num{rv.ts.decider.doneneutral.ecescaledhi}]}} & \num{rv.ts.decider.dtwo.ece} & \num{rv.ts.decider.dtwo.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.decider.dtwo.ecescaledlo}, \num{rv.ts.decider.dtwo.ecescaledhi}]}} & \num{rv.ts.decider.toxicity.ece} & \num{rv.ts.decider.toxicity.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.decider.toxicity.ecescaledlo}, \num{rv.ts.decider.toxicity.ecescaledhi}]}} & \num{rv.ts.decider.power.ece} & \num{rv.ts.decider.power.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.decider.power.ecescaledlo}, \num{rv.ts.decider.power.ecescaledhi}]}} & \best{\num{rv.ts.decider.emotion.ece}} & \best{\num{rv.ts.decider.emotion.ecescaled}}\par{\scriptsize\cellnote{[\num{rv.ts.decider.emotion.ecescaledlo}, \num{rv.ts.decider.emotion.ecescaledhi}]}} & \num{rv.ts.decider.politeness.ece} & \num{rv.ts.decider.politeness.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.decider.politeness.ecescaledlo}, \num{rv.ts.decider.politeness.ecescaledhi}]}} \\
\msw{thisthat}this-that-model-1.0 & \num{rv.ts.thisthat.doneneutral.ece} & \num{rv.ts.thisthat.doneneutral.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.thisthat.doneneutral.ecescaledlo}, \num{rv.ts.thisthat.doneneutral.ecescaledhi}]}} & \num{rv.ts.thisthat.dtwo.ece} & \best{\num{rv.ts.thisthat.dtwo.ecescaled}}\par{\scriptsize\cellnote{[\num{rv.ts.thisthat.dtwo.ecescaledlo}, \num{rv.ts.thisthat.dtwo.ecescaledhi}]}} & \num{rv.ts.thisthat.toxicity.ece} & \num{rv.ts.thisthat.toxicity.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.thisthat.toxicity.ecescaledlo}, \num{rv.ts.thisthat.toxicity.ecescaledhi}]}} & \num{rv.ts.thisthat.power.ece} & \best{\num{rv.ts.thisthat.power.ecescaled}}\par{\scriptsize\cellnote{[\num{rv.ts.thisthat.power.ecescaledlo}, \num{rv.ts.thisthat.power.ecescaledhi}]}} & \num{rv.ts.thisthat.emotion.ece} & \num{rv.ts.thisthat.emotion.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.thisthat.emotion.ecescaledlo}, \num{rv.ts.thisthat.emotion.ecescaledhi}]}} & \num{rv.ts.thisthat.politeness.ece} & \num{rv.ts.thisthat.politeness.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.thisthat.politeness.ecescaledlo}, \num{rv.ts.thisthat.politeness.ecescaledhi}]}} \\
\msw{nimble}Nimble-9B & \num{rv.ts.nimble.doneneutral.ece} & \best{\num{rv.ts.nimble.doneneutral.ecescaled}}\par{\scriptsize\cellnote{[\num{rv.ts.nimble.doneneutral.ecescaledlo}, \num{rv.ts.nimble.doneneutral.ecescaledhi}]}} & \num{rv.ts.nimble.dtwo.ece} & \num{rv.ts.nimble.dtwo.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.nimble.dtwo.ecescaledlo}, \num{rv.ts.nimble.dtwo.ecescaledhi}]}} & \num{rv.ts.nimble.toxicity.ece} & \num{rv.ts.nimble.toxicity.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.nimble.toxicity.ecescaledlo}, \num{rv.ts.nimble.toxicity.ecescaledhi}]}} & \num{rv.ts.nimble.power.ece} & \num{rv.ts.nimble.power.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.nimble.power.ecescaledlo}, \num{rv.ts.nimble.power.ecescaledhi}]}} & \num{rv.ts.nimble.emotion.ece} & \num{rv.ts.nimble.emotion.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.nimble.emotion.ecescaledlo}, \num{rv.ts.nimble.emotion.ecescaledhi}]}} & \num{rv.ts.nimble.politeness.ece} & \num{rv.ts.nimble.politeness.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.nimble.politeness.ecescaledlo}, \num{rv.ts.nimble.politeness.ecescaledhi}]}} \\
\groupspan{thirteen}{Generative comparators}
\msw{compopen}Qwen3-14B, verbal & \num{rv.ts.compopen.doneneutral.ece} & \num{rv.ts.compopen.doneneutral.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.compopen.doneneutral.ecescaledlo}, \num{rv.ts.compopen.doneneutral.ecescaledhi}]}} & \num{rv.ts.compopen.dtwo.ece} & \num{rv.ts.compopen.dtwo.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.compopen.dtwo.ecescaledlo}, \num{rv.ts.compopen.dtwo.ecescaledhi}]}} & \num{rv.ts.compopen.toxicity.ece} & \num{rv.ts.compopen.toxicity.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.compopen.toxicity.ecescaledlo}, \num{rv.ts.compopen.toxicity.ecescaledhi}]}} & \num{rv.ts.compopen.power.ece} & \num{rv.ts.compopen.power.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.compopen.power.ecescaledlo}, \num{rv.ts.compopen.power.ecescaledhi}]}} & \num{rv.ts.compopen.emotion.ece} & \num{rv.ts.compopen.emotion.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.compopen.emotion.ecescaledlo}, \num{rv.ts.compopen.emotion.ecescaledhi}]}} & \num{rv.ts.compopen.politeness.ece} & \num{rv.ts.compopen.politeness.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.compopen.politeness.ecescaledlo}, \num{rv.ts.compopen.politeness.ecescaledhi}]}} \\
\addlinespace[2.5pt]
\msw{comptwo}Qwen3.6-27B, verbal & \num{rv.ts.comptwo.doneneutral.ece} & \num{rv.ts.comptwo.doneneutral.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.comptwo.doneneutral.ecescaledlo}, \num{rv.ts.comptwo.doneneutral.ecescaledhi}]}} & \num{rv.ts.comptwo.dtwo.ece} & \num{rv.ts.comptwo.dtwo.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.comptwo.dtwo.ecescaledlo}, \num{rv.ts.comptwo.dtwo.ecescaledhi}]}} & \num{rv.ts.comptwo.toxicity.ece} & \num{rv.ts.comptwo.toxicity.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.comptwo.toxicity.ecescaledlo}, \num{rv.ts.comptwo.toxicity.ecescaledhi}]}} & \num{rv.ts.comptwo.power.ece} & \num{rv.ts.comptwo.power.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.comptwo.power.ecescaledlo}, \num{rv.ts.comptwo.power.ecescaledhi}]}} & \num{rv.ts.comptwo.emotion.ece} & \num{rv.ts.comptwo.emotion.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.comptwo.emotion.ecescaledlo}, \num{rv.ts.comptwo.emotion.ecescaledhi}]}} & \num{rv.ts.comptwo.politeness.ece} & \num{rv.ts.comptwo.politeness.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.comptwo.politeness.ecescaledlo}, \num{rv.ts.comptwo.politeness.ecescaledhi}]}} \\
\msw{comptwoll}Qwen3.6-27B, likelihood & \num{rv.ts.comptwoll.doneneutral.ece} & \num{rv.ts.comptwoll.doneneutral.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.comptwoll.doneneutral.ecescaledlo}, \num{rv.ts.comptwoll.doneneutral.ecescaledhi}]}} & \num{rv.ts.comptwoll.dtwo.ece} & \num{rv.ts.comptwoll.dtwo.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.comptwoll.dtwo.ecescaledlo}, \num{rv.ts.comptwoll.dtwo.ecescaledhi}]}} & \num{rv.ts.comptwoll.toxicity.ece} & \num{rv.ts.comptwoll.toxicity.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.comptwoll.toxicity.ecescaledlo}, \num{rv.ts.comptwoll.toxicity.ecescaledhi}]}} & \num{rv.ts.comptwoll.power.ece} & \num{rv.ts.comptwoll.power.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.comptwoll.power.ecescaledlo}, \num{rv.ts.comptwoll.power.ecescaledhi}]}} & \num{rv.ts.comptwoll.emotion.ece} & \num{rv.ts.comptwoll.emotion.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.comptwoll.emotion.ecescaledlo}, \num{rv.ts.comptwoll.emotion.ecescaledhi}]}} & \num{rv.ts.comptwoll.politeness.ece} & \num{rv.ts.comptwoll.politeness.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.comptwoll.politeness.ecescaledlo}, \num{rv.ts.comptwoll.politeness.ecescaledhi}]}} \\
\msw{comptwothink}Qwen3.6-27B, thinking & \num{rv.ts.comptwothink.doneneutral.ece} & \num{rv.ts.comptwothink.doneneutral.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.comptwothink.doneneutral.ecescaledlo}, \num{rv.ts.comptwothink.doneneutral.ecescaledhi}]}} & \num{rv.ts.comptwothink.dtwo.ece} & \num{rv.ts.comptwothink.dtwo.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.comptwothink.dtwo.ecescaledlo}, \num{rv.ts.comptwothink.dtwo.ecescaledhi}]}} & \num{rv.ts.comptwothink.toxicity.ece} & \num{rv.ts.comptwothink.toxicity.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.comptwothink.toxicity.ecescaledlo}, \num{rv.ts.comptwothink.toxicity.ecescaledhi}]}} & \num{rv.ts.comptwothink.power.ece} & \num{rv.ts.comptwothink.power.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.comptwothink.power.ecescaledlo}, \num{rv.ts.comptwothink.power.ecescaledhi}]}} & \num{rv.ts.comptwothink.emotion.ece} & \num{rv.ts.comptwothink.emotion.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.comptwothink.emotion.ecescaledlo}, \num{rv.ts.comptwothink.emotion.ecescaledhi}]}} & \num{rv.ts.comptwothink.politeness.ece} & \num{rv.ts.comptwothink.politeness.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.comptwothink.politeness.ecescaledlo}, \num{rv.ts.comptwothink.politeness.ecescaledhi}]}} \\
\addlinespace[2.5pt]
\msw{compgem}Gemma-4-31B, verbal & \num{rv.ts.compgem.doneneutral.ece} & \num{rv.ts.compgem.doneneutral.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.compgem.doneneutral.ecescaledlo}, \num{rv.ts.compgem.doneneutral.ecescaledhi}]}} & \best{\num{rv.ts.compgem.dtwo.ece}} & \num{rv.ts.compgem.dtwo.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.compgem.dtwo.ecescaledlo}, \num{rv.ts.compgem.dtwo.ecescaledhi}]}} & \num{rv.ts.compgem.toxicity.ece} & \num{rv.ts.compgem.toxicity.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.compgem.toxicity.ecescaledlo}, \num{rv.ts.compgem.toxicity.ecescaledhi}]}} & \num{rv.ts.compgem.power.ece} & \num{rv.ts.compgem.power.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.compgem.power.ecescaledlo}, \num{rv.ts.compgem.power.ecescaledhi}]}} & \num{rv.ts.compgem.emotion.ece} & \num{rv.ts.compgem.emotion.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.compgem.emotion.ecescaledlo}, \num{rv.ts.compgem.emotion.ecescaledhi}]}} & \num{rv.ts.compgem.politeness.ece} & \num{rv.ts.compgem.politeness.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.compgem.politeness.ecescaledlo}, \num{rv.ts.compgem.politeness.ecescaledhi}]}} \\
\msw{compgemll}Gemma-4-31B, likelihood & \num{rv.ts.compgemll.doneneutral.ece} & \num{rv.ts.compgemll.doneneutral.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.compgemll.doneneutral.ecescaledlo}, \num{rv.ts.compgemll.doneneutral.ecescaledhi}]}} & \num{rv.ts.compgemll.dtwo.ece} & \num{rv.ts.compgemll.dtwo.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.compgemll.dtwo.ecescaledlo}, \num{rv.ts.compgemll.dtwo.ecescaledhi}]}} & \num{rv.ts.compgemll.toxicity.ece} & \num{rv.ts.compgemll.toxicity.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.compgemll.toxicity.ecescaledlo}, \num{rv.ts.compgemll.toxicity.ecescaledhi}]}} & \num{rv.ts.compgemll.power.ece} & \num{rv.ts.compgemll.power.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.compgemll.power.ecescaledlo}, \num{rv.ts.compgemll.power.ecescaledhi}]}} & \num{rv.ts.compgemll.emotion.ece} & \num{rv.ts.compgemll.emotion.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.compgemll.emotion.ecescaledlo}, \num{rv.ts.compgemll.emotion.ecescaledhi}]}} & \num{rv.ts.compgemll.politeness.ece} & \num{rv.ts.compgemll.politeness.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.compgemll.politeness.ecescaledlo}, \num{rv.ts.compgemll.politeness.ecescaledhi}]}} \\*
\addlinespace[2.5pt]
\msw{compmis}Mistral-Small-24B, verbal & \num{rv.ts.compmis.doneneutral.ece} & \num{rv.ts.compmis.doneneutral.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.compmis.doneneutral.ecescaledlo}, \num{rv.ts.compmis.doneneutral.ecescaledhi}]}} & \num{rv.ts.compmis.dtwo.ece} & \num{rv.ts.compmis.dtwo.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.compmis.dtwo.ecescaledlo}, \num{rv.ts.compmis.dtwo.ecescaledhi}]}} & \num{rv.ts.compmis.toxicity.ece} & \num{rv.ts.compmis.toxicity.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.compmis.toxicity.ecescaledlo}, \num{rv.ts.compmis.toxicity.ecescaledhi}]}} & \num{rv.ts.compmis.power.ece} & \num{rv.ts.compmis.power.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.compmis.power.ecescaledlo}, \num{rv.ts.compmis.power.ecescaledhi}]}} & \num{rv.ts.compmis.emotion.ece} & \num{rv.ts.compmis.emotion.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.compmis.emotion.ecescaledlo}, \num{rv.ts.compmis.emotion.ecescaledhi}]}} & \num{rv.ts.compmis.politeness.ece} & \num{rv.ts.compmis.politeness.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.compmis.politeness.ecescaledlo}, \num{rv.ts.compmis.politeness.ecescaledhi}]}} \\*
\msw{compmisll}Mistral-Small-24B, likelihood & \num{rv.ts.compmisll.doneneutral.ece} & \num{rv.ts.compmisll.doneneutral.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.compmisll.doneneutral.ecescaledlo}, \num{rv.ts.compmisll.doneneutral.ecescaledhi}]}} & \num{rv.ts.compmisll.dtwo.ece} & \num{rv.ts.compmisll.dtwo.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.compmisll.dtwo.ecescaledlo}, \num{rv.ts.compmisll.dtwo.ecescaledhi}]}} & \num{rv.ts.compmisll.toxicity.ece} & \num{rv.ts.compmisll.toxicity.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.compmisll.toxicity.ecescaledlo}, \num{rv.ts.compmisll.toxicity.ecescaledhi}]}} & \num{rv.ts.compmisll.power.ece} & \num{rv.ts.compmisll.power.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.compmisll.power.ecescaledlo}, \num{rv.ts.compmisll.power.ecescaledhi}]}} & \num{rv.ts.compmisll.emotion.ece} & \num{rv.ts.compmisll.emotion.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.compmisll.emotion.ecescaledlo}, \num{rv.ts.compmisll.emotion.ecescaledhi}]}} & \best{\num{rv.ts.compmisll.politeness.ece}} & \num{rv.ts.compmisll.politeness.ecescaled}\par{\scriptsize\cellnote{[\num{rv.ts.compmisll.politeness.ecescaledlo}, \num{rv.ts.compmisll.politeness.ecescaledhi}]}} \\*
\bottomrule
\end{tabular}
\tablenote{Ship.\ is the expected calibration error as shipped and Scaled the error after temperature scaling, with one temperature per question type fitted on the calibration split for D1 and temperatures cross-fitted over item folds for the other tasks. Beneath each scaled error is its cluster bootstrap interval at \num{p.boot.level} percent, whose \num{p.boot.refitreps} replicates refit the temperatures. Bold marks the lowest error in each column, with ties bolded.}


==> tables/t10_selective.tex <==
% Generated by shared/src/t01_tables.py. Do not edit by hand.
% Every numeric cell is a num-macro from numbers.tex; -- means that
% model has no result for this cell yet. Needs paper4a_tables.sty.
\tablestyle
\begin{tabular}{P{0.2850}N{0.0894}N{0.0894}N{0.0894}N{0.0894}N{0.0894}N{0.0894}N{0.0894}N{0.0894}}
\toprule
\headrow \hdtop{} & \hdgroup{four}{D1 typed-decisions} & \hdgroup{four}{D2 CLINC-150} \\
\bandrules{2-5,6-9}
\headrow \hdsub{Model} & \hdsub{In-sample} & \hdsub{Held-out} & \hdsub{Risk} & \hdsub{Bound} & \hdsub{In-sample} & \hdsub{Held-out} & \hdsub{Risk} & \hdsub{Bound} \\
\midrule
\tabhead
\groupspan{nine}{Hosted}
\msw{jev}Jev 1.13.0 & \num{rv.sel.jev.doneneutral.covfive}\par{\scriptsize\cellnote{[\num{rv.sel.jev.doneneutral.covfivelo}, \num{rv.sel.jev.doneneutral.covfivehi}]}} & \num{rv.ho.jev.doneneutral.five.cov} & \num{rv.ho.jev.doneneutral.five.risk} & \num{rv.ho.jev.doneneutral.five.riskub} & \num{rv.sel.jev.dtwo.covfive}\par{\scriptsize\cellnote{[\num{rv.sel.jev.dtwo.covfivelo}, \num{rv.sel.jev.dtwo.covfivehi}]}} & \num{rv.ho.jev.dtwo.five.cov} & \num{rv.ho.jev.dtwo.five.risk} & \num{rv.ho.jev.dtwo.five.riskub} \\
\groupspan{nine}{Open, encoder head}
\msw{layaen}Laya (English) & \num{rv.sel.layaen.doneneutral.covfive}\par{\scriptsize\cellnote{[\num{rv.sel.layaen.doneneutral.covfivelo}, \num{rv.sel.layaen.doneneutral.covfivehi}]}} & \num{rv.ho.layaen.doneneutral.five.cov} & \num{rv.ho.layaen.doneneutral.five.risk} & \num{rv.ho.layaen.doneneutral.five.riskub} & -- & -- & -- & -- \\
\msw{layaml}Laya (multilingual) & \num{rv.sel.layaml.doneneutral.covfive}\par{\scriptsize\cellnote{[\num{rv.sel.layaml.doneneutral.covfivelo}, \num{rv.sel.layaml.doneneutral.covfivehi}]}} & \num{rv.ho.layaml.doneneutral.five.cov} & \num{rv.ho.layaml.doneneutral.five.risk} & \num{rv.ho.layaml.doneneutral.five.riskub} & \num{rv.sel.layaml.dtwo.covfive}\par{\scriptsize\cellnote{[\num{rv.sel.layaml.dtwo.covfivelo}, \num{rv.sel.layaml.dtwo.covfivehi}]}} & \num{rv.ho.layaml.dtwo.five.cov} & -- & -- \\
\groupspan{nine}{Open, decoder head}
\msw{kevsmall}Kev-0.8B & \num{rv.sel.kevsmall.doneneutral.covfive}\par{\scriptsize\cellnote{[\num{rv.sel.kevsmall.doneneutral.covfivelo}, \num{rv.sel.kevsmall.doneneutral.covfivehi}]}} & \num{rv.ho.kevsmall.doneneutral.five.cov} & \num{rv.ho.kevsmall.doneneutral.five.risk} & \num{rv.ho.kevsmall.doneneutral.five.riskub} & \num{rv.sel.kevsmall.dtwo.covfive}\par{\scriptsize\cellnote{[\num{rv.sel.kevsmall.dtwo.covfivelo}, \num{rv.sel.kevsmall.dtwo.covfivehi}]}} & \num{rv.ho.kevsmall.dtwo.five.cov} & \num{rv.ho.kevsmall.dtwo.five.risk} & \num{rv.ho.kevsmall.dtwo.five.riskub} \\
\msw{kevlarge}Kev-9B & \num{rv.sel.kevlarge.doneneutral.covfive}\par{\scriptsize\cellnote{[\num{rv.sel.kevlarge.doneneutral.covfivelo}, \num{rv.sel.kevlarge.doneneutral.covfivehi}]}} & \num{rv.ho.kevlarge.doneneutral.five.cov} & \num{rv.ho.kevlarge.doneneutral.five.risk} & \num{rv.ho.kevlarge.doneneutral.five.riskub} & \num{rv.sel.kevlarge.dtwo.covfive}\par{\scriptsize\cellnote{[\num{rv.sel.kevlarge.dtwo.covfivelo}, \num{rv.sel.kevlarge.dtwo.covfivehi}]}} & \num{rv.ho.kevlarge.dtwo.five.cov} & \num{rv.ho.kevlarge.dtwo.five.risk} & \num{rv.ho.kevlarge.dtwo.five.riskub} \\
\msw{decider}decider-2b & \num{rv.sel.decider.doneneutral.covfive}\par{\scriptsize\cellnote{[\num{rv.sel.decider.doneneutral.covfivelo}, \num{rv.sel.decider.doneneutral.covfivehi}]}} & \num{rv.ho.decider.doneneutral.five.cov} & \num{rv.ho.decider.doneneutral.five.risk} & \num{rv.ho.decider.doneneutral.five.riskub} & \num{rv.sel.decider.dtwo.covfive}\par{\scriptsize\cellnote{[\num{rv.sel.decider.dtwo.covfivelo}, \num{rv.sel.decider.dtwo.covfivehi}]}} & \num{rv.ho.decider.dtwo.five.cov} & \num{rv.ho.decider.dtwo.five.risk} & \num{rv.ho.decider.dtwo.five.riskub} \\
\msw{thisthat}this-that-model-1.0 & \num{rv.sel.thisthat.doneneutral.covfive}\par{\scriptsize\cellnote{[\num{rv.sel.thisthat.doneneutral.covfivelo}, \num{rv.sel.thisthat.doneneutral.covfivehi}]}} & \num{rv.ho.thisthat.doneneutral.five.cov} & \num{rv.ho.thisthat.doneneutral.five.risk} & \num{rv.ho.thisthat.doneneutral.five.riskub} & \num{rv.sel.thisthat.dtwo.covfive}\par{\scriptsize\cellnote{[\num{rv.sel.thisthat.dtwo.covfivelo}, \num{rv.sel.thisthat.dtwo.covfivehi}]}} & \num{rv.ho.thisthat.dtwo.five.cov} & \num{rv.ho.thisthat.dtwo.five.risk} & \num{rv.ho.thisthat.dtwo.five.riskub} \\
\msw{nimble}Nimble-9B & \num{rv.sel.nimble.doneneutral.covfive}\par{\scriptsize\cellnote{[\num{rv.sel.nimble.doneneutral.covfivelo}, \num{rv.sel.nimble.doneneutral.covfivehi}]}} & \num{rv.ho.nimble.doneneutral.five.cov} & \num{rv.ho.nimble.doneneutral.five.risk} & \num{rv.ho.nimble.doneneutral.five.riskub} & \num{rv.sel.nimble.dtwo.covfive}\par{\scriptsize\cellnote{[\num{rv.sel.nimble.dtwo.covfivelo}, \num{rv.sel.nimble.dtwo.covfivehi}]}} & \num{rv.ho.nimble.dtwo.five.cov} & \num{rv.ho.nimble.dtwo.five.risk} & \num{rv.ho.nimble.dtwo.five.riskub} \\
\groupspan{nine}{Generative comparators}
\msw{compopen}Qwen3-14B, verbal & \num{rv.sel.compopen.doneneutral.covfive}\par{\scriptsize\cellnote{[\num{rv.sel.compopen.doneneutral.covfivelo}, \num{rv.sel.compopen.doneneutral.covfivehi}]}} & \num{rv.ho.compopen.doneneutral.five.cov} & \num{rv.ho.compopen.doneneutral.five.risk} & \num{rv.ho.compopen.doneneutral.five.riskub} & \num{rv.sel.compopen.dtwo.covfive}\par{\scriptsize\cellnote{[\num{rv.sel.compopen.dtwo.covfivelo}, \num{rv.sel.compopen.dtwo.covfivehi}]}} & \num{rv.ho.compopen.dtwo.five.cov} & \num{rv.ho.compopen.dtwo.five.risk} & \num{rv.ho.compopen.dtwo.five.riskub} \\
\addlinespace[2.5pt]
\msw{comptwo}Qwen3.6-27B, verbal & \num{rv.sel.comptwo.doneneutral.covfive}\par{\scriptsize\cellnote{[\num{rv.sel.comptwo.doneneutral.covfivelo}, \num{rv.sel.comptwo.doneneutral.covfivehi}]}} & \num{rv.ho.comptwo.doneneutral.five.cov} & -- & -- & \num{rv.sel.comptwo.dtwo.covfive}\par{\scriptsize\cellnote{[\num{rv.sel.comptwo.dtwo.covfivelo}, \num{rv.sel.comptwo.dtwo.covfivehi}]}} & \num{rv.ho.comptwo.dtwo.five.cov} & \num{rv.ho.comptwo.dtwo.five.risk} & \num{rv.ho.comptwo.dtwo.five.riskub} \\
\msw{comptwoll}Qwen3.6-27B, likelihood & \num{rv.sel.comptwoll.doneneutral.covfive}\par{\scriptsize\cellnote{[\num{rv.sel.comptwoll.doneneutral.covfivelo}, \num{rv.sel.comptwoll.doneneutral.covfivehi}]}} & \best{\num{rv.ho.comptwoll.doneneutral.five.cov}} & \num{rv.ho.comptwoll.doneneutral.five.risk} & \num{rv.ho.comptwoll.doneneutral.five.riskub} & \num{rv.sel.comptwoll.dtwo.covfive}\par{\scriptsize\cellnote{[\num{rv.sel.comptwoll.dtwo.covfivelo}, \num{rv.sel.comptwoll.dtwo.covfivehi}]}} & \num{rv.ho.comptwoll.dtwo.five.cov} & \num{rv.ho.comptwoll.dtwo.five.risk} & \num{rv.ho.comptwoll.dtwo.five.riskub} \\
\msw{comptwothink}Qwen3.6-27B, thinking & \num{rv.sel.comptwothink.doneneutral.covfive}\par{\scriptsize\cellnote{[\num{rv.sel.comptwothink.doneneutral.covfivelo}, \num{rv.sel.comptwothink.doneneutral.covfivehi}]}} & \num{rv.ho.comptwothink.doneneutral.five.cov} & \num{rv.ho.comptwothink.doneneutral.five.risk} & \num{rv.ho.comptwothink.doneneutral.five.riskub} & \num{rv.sel.comptwothink.dtwo.covfive}\par{\scriptsize\cellnote{[\num{rv.sel.comptwothink.dtwo.covfivelo}, \num{rv.sel.comptwothink.dtwo.covfivehi}]}} & \num{rv.ho.comptwothink.dtwo.five.cov} & \num{rv.ho.comptwothink.dtwo.five.risk} & \num{rv.ho.comptwothink.dtwo.five.riskub} \\
\addlinespace[2.5pt]
\msw{compgem}Gemma-4-31B, verbal & \num{rv.sel.compgem.doneneutral.covfive}\par{\scriptsize\cellnote{[\num{rv.sel.compgem.doneneutral.covfivelo}, \num{rv.sel.compgem.doneneutral.covfivehi}]}} & \num{rv.ho.compgem.doneneutral.five.cov} & \num{rv.ho.compgem.doneneutral.five.risk} & \num{rv.ho.compgem.doneneutral.five.riskub} & \num{rv.sel.compgem.dtwo.covfive}\par{\scriptsize\cellnote{[\num{rv.sel.compgem.dtwo.covfivelo}, \num{rv.sel.compgem.dtwo.covfivehi}]}} & \num{rv.ho.compgem.dtwo.five.cov} & \num{rv.ho.compgem.dtwo.five.risk} & \num{rv.ho.compgem.dtwo.five.riskub} \\
\msw{compgemll}Gemma-4-31B, likelihood & \num{rv.sel.compgemll.doneneutral.covfive}\par{\scriptsize\cellnote{[\num{rv.sel.compgemll.doneneutral.covfivelo}, \num{rv.sel.compgemll.doneneutral.covfivehi}]}} & \num{rv.ho.compgemll.doneneutral.five.cov} & \num{rv.ho.compgemll.doneneutral.five.risk} & \num{rv.ho.compgemll.doneneutral.five.riskub} & \num{rv.sel.compgemll.dtwo.covfive}\par{\scriptsize\cellnote{[\num{rv.sel.compgemll.dtwo.covfivelo}, \num{rv.sel.compgemll.dtwo.covfivehi}]}} & \best{\num{rv.ho.compgemll.dtwo.five.cov}} & \num{rv.ho.compgemll.dtwo.five.risk} & \num{rv.ho.compgemll.dtwo.five.riskub} \\*
\addlinespace[2.5pt]
\msw{compmis}Mistral-Small-24B, verbal & \num{rv.sel.compmis.doneneutral.covfive}\par{\scriptsize\cellnote{[\num{rv.sel.compmis.doneneutral.covfivelo}, \num{rv.sel.compmis.doneneutral.covfivehi}]}} & \num{rv.ho.compmis.doneneutral.five.cov} & -- & -- & \num{rv.sel.compmis.dtwo.covfive}\par{\scriptsize\cellnote{[\num{rv.sel.compmis.dtwo.covfivelo}, \num{rv.sel.compmis.dtwo.covfivehi}]}} & \num{rv.ho.compmis.dtwo.five.cov} & -- & -- \\*
\msw{compmisll}Mistral-Small-24B, likelihood & \num{rv.sel.compmisll.doneneutral.covfive}\par{\scriptsize\cellnote{[\num{rv.sel.compmisll.doneneutral.covfivelo}, \num{rv.sel.compmisll.doneneutral.covfivehi}]}} & \num{rv.ho.compmisll.doneneutral.five.cov} & \num{rv.ho.compmisll.doneneutral.five.risk} & \num{rv.ho.compmisll.doneneutral.five.riskub} & \num{rv.sel.compmisll.dtwo.covfive}\par{\scriptsize\cellnote{[\num{rv.sel.compmisll.dtwo.covfivelo}, \num{rv.sel.compmisll.dtwo.covfivehi}]}} & \num{rv.ho.compmisll.dtwo.five.cov} & \num{rv.ho.compmisll.dtwo.five.risk} & \num{rv.ho.compmisll.dtwo.five.riskub} \\*
\bottomrule
\end{tabular}
\tablenote{In-sample is the coverage at \num{p.riskfive} percent risk with the threshold chosen on the scored decisions, with its cluster bootstrap interval at \num{p.boot.level} percent beneath. Held-out applies a threshold chosen by the same rule on the calibration split for D1 and on the other item folds for D2. Risk is the error rate of the decisions it accepts and Bound is the one-sided \num{p.boot.level} percent Clopper-Pearson upper limit of that rate, with a dash where no decision is accepted. A coverage printed as zero can still accept a few decisions. Bold marks the highest held-out coverage on each dataset, with ties bolded.}


==> tables/t11_paired.tex <==
% Generated by shared/src/t01_tables.py. Do not edit by hand.
% Every numeric cell is a num-macro from numbers.tex; -- means that
% model has no result for this cell yet. Needs paper4a_tables.sty.
\tablestyle
\begin{tabular}{P{0.2850}N{0.1192}N{0.1192}N{0.1192}N{0.1192}N{0.1192}N{0.1192}}
\toprule
\headrow \hdtop{} & \hdgroup{two}{Workflow and intent sets} & \hdgroup{four}{D3 social science tasks} \\
\bandrules{2-3,4-7}
\headrow \hdsub{Model} & \hdsub{D1} & \hdsub{D2} & \hdsub{Derail.} & \hdsub{Power} & \hdsub{Emotion} & \hdsub{Polite.} \\
\midrule
\tabhead
\groupspan{seven}{Open, encoder head}
\msw{layaen}Laya (English) & \best{\num{rv.pd.layaen.doneneutral.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.layaen.doneneutral.difflo}, \num{rv.pd.layaen.doneneutral.diffhi}]}} & -- & \num{rv.pd.layaen.toxicity.diff}\par{\scriptsize\cellnote{[\num{rv.pd.layaen.toxicity.difflo}, \num{rv.pd.layaen.toxicity.diffhi}]}} & \best{\num{rv.pd.layaen.power.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.layaen.power.difflo}, \num{rv.pd.layaen.power.diffhi}]}} & \num{rv.pd.layaen.emotion.diff}\par{\scriptsize\cellnote{[\num{rv.pd.layaen.emotion.difflo}, \num{rv.pd.layaen.emotion.diffhi}]}} & \best{\num{rv.pd.layaen.politeness.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.layaen.politeness.difflo}, \num{rv.pd.layaen.politeness.diffhi}]}} \\
\msw{layaml}Laya (multilingual) & \best{\num{rv.pd.layaml.doneneutral.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.layaml.doneneutral.difflo}, \num{rv.pd.layaml.doneneutral.diffhi}]}} & \best{\num{rv.pd.layaml.dtwo.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.layaml.dtwo.difflo}, \num{rv.pd.layaml.dtwo.diffhi}]}} & \num{rv.pd.layaml.toxicity.diff}\par{\scriptsize\cellnote{[\num{rv.pd.layaml.toxicity.difflo}, \num{rv.pd.layaml.toxicity.diffhi}]}} & \best{\num{rv.pd.layaml.power.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.layaml.power.difflo}, \num{rv.pd.layaml.power.diffhi}]}} & \best{\num{rv.pd.layaml.emotion.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.layaml.emotion.difflo}, \num{rv.pd.layaml.emotion.diffhi}]}} & \best{\num{rv.pd.layaml.politeness.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.layaml.politeness.difflo}, \num{rv.pd.layaml.politeness.diffhi}]}} \\
\groupspan{seven}{Open, decoder head}
\msw{kevsmall}Kev-0.8B & \best{\num{rv.pd.kevsmall.doneneutral.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.kevsmall.doneneutral.difflo}, \num{rv.pd.kevsmall.doneneutral.diffhi}]}} & \best{\num{rv.pd.kevsmall.dtwo.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.kevsmall.dtwo.difflo}, \num{rv.pd.kevsmall.dtwo.diffhi}]}} & \num{rv.pd.kevsmall.toxicity.diff}\par{\scriptsize\cellnote{[\num{rv.pd.kevsmall.toxicity.difflo}, \num{rv.pd.kevsmall.toxicity.diffhi}]}} & \best{\num{rv.pd.kevsmall.power.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.kevsmall.power.difflo}, \num{rv.pd.kevsmall.power.diffhi}]}} & \num{rv.pd.kevsmall.emotion.diff}\par{\scriptsize\cellnote{[\num{rv.pd.kevsmall.emotion.difflo}, \num{rv.pd.kevsmall.emotion.diffhi}]}} & \best{\num{rv.pd.kevsmall.politeness.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.kevsmall.politeness.difflo}, \num{rv.pd.kevsmall.politeness.diffhi}]}} \\
\msw{kevlarge}Kev-9B & \num{rv.pd.kevlarge.doneneutral.diff}\par{\scriptsize\cellnote{[\num{rv.pd.kevlarge.doneneutral.difflo}, \num{rv.pd.kevlarge.doneneutral.diffhi}]}} & \best{\num{rv.pd.kevlarge.dtwo.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.kevlarge.dtwo.difflo}, \num{rv.pd.kevlarge.dtwo.diffhi}]}} & \num{rv.pd.kevlarge.toxicity.diff}\par{\scriptsize\cellnote{[\num{rv.pd.kevlarge.toxicity.difflo}, \num{rv.pd.kevlarge.toxicity.diffhi}]}} & \num{rv.pd.kevlarge.power.diff}\par{\scriptsize\cellnote{[\num{rv.pd.kevlarge.power.difflo}, \num{rv.pd.kevlarge.power.diffhi}]}} & \num{rv.pd.kevlarge.emotion.diff}\par{\scriptsize\cellnote{[\num{rv.pd.kevlarge.emotion.difflo}, \num{rv.pd.kevlarge.emotion.diffhi}]}} & \best{\num{rv.pd.kevlarge.politeness.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.kevlarge.politeness.difflo}, \num{rv.pd.kevlarge.politeness.diffhi}]}} \\
\msw{decider}decider-2b & \best{\num{rv.pd.decider.doneneutral.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.decider.doneneutral.difflo}, \num{rv.pd.decider.doneneutral.diffhi}]}} & \best{\num{rv.pd.decider.dtwo.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.decider.dtwo.difflo}, \num{rv.pd.decider.dtwo.diffhi}]}} & \best{\num{rv.pd.decider.toxicity.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.decider.toxicity.difflo}, \num{rv.pd.decider.toxicity.diffhi}]}} & \best{\num{rv.pd.decider.power.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.decider.power.difflo}, \num{rv.pd.decider.power.diffhi}]}} & \best{\num{rv.pd.decider.emotion.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.decider.emotion.difflo}, \num{rv.pd.decider.emotion.diffhi}]}} & \best{\num{rv.pd.decider.politeness.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.decider.politeness.difflo}, \num{rv.pd.decider.politeness.diffhi}]}} \\
\msw{thisthat}this-that-model-1.0 & \best{\num{rv.pd.thisthat.doneneutral.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.thisthat.doneneutral.difflo}, \num{rv.pd.thisthat.doneneutral.diffhi}]}} & \best{\num{rv.pd.thisthat.dtwo.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.thisthat.dtwo.difflo}, \num{rv.pd.thisthat.dtwo.diffhi}]}} & \best{\num{rv.pd.thisthat.toxicity.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.thisthat.toxicity.difflo}, \num{rv.pd.thisthat.toxicity.diffhi}]}} & \best{\num{rv.pd.thisthat.power.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.thisthat.power.difflo}, \num{rv.pd.thisthat.power.diffhi}]}} & \best{\num{rv.pd.thisthat.emotion.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.thisthat.emotion.difflo}, \num{rv.pd.thisthat.emotion.diffhi}]}} & \best{\num{rv.pd.thisthat.politeness.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.thisthat.politeness.difflo}, \num{rv.pd.thisthat.politeness.diffhi}]}} \\
\msw{nimble}Nimble-9B & \best{\num{rv.pd.nimble.doneneutral.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.nimble.doneneutral.difflo}, \num{rv.pd.nimble.doneneutral.diffhi}]}} & \best{\num{rv.pd.nimble.dtwo.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.nimble.dtwo.difflo}, \num{rv.pd.nimble.dtwo.diffhi}]}} & \num{rv.pd.nimble.toxicity.diff}\par{\scriptsize\cellnote{[\num{rv.pd.nimble.toxicity.difflo}, \num{rv.pd.nimble.toxicity.diffhi}]}} & \num{rv.pd.nimble.power.diff}\par{\scriptsize\cellnote{[\num{rv.pd.nimble.power.difflo}, \num{rv.pd.nimble.power.diffhi}]}} & \num{rv.pd.nimble.emotion.diff}\par{\scriptsize\cellnote{[\num{rv.pd.nimble.emotion.difflo}, \num{rv.pd.nimble.emotion.diffhi}]}} & \best{\num{rv.pd.nimble.politeness.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.nimble.politeness.difflo}, \num{rv.pd.nimble.politeness.diffhi}]}} \\
\groupspan{seven}{Generative comparators}
\msw{compopen}Qwen3-14B, verbal & \best{\num{rv.pd.compopen.doneneutral.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.compopen.doneneutral.difflo}, \num{rv.pd.compopen.doneneutral.diffhi}]}} & \best{\num{rv.pd.compopen.dtwo.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.compopen.dtwo.difflo}, \num{rv.pd.compopen.dtwo.diffhi}]}} & \num{rv.pd.compopen.toxicity.diff}\par{\scriptsize\cellnote{[\num{rv.pd.compopen.toxicity.difflo}, \num{rv.pd.compopen.toxicity.diffhi}]}} & \num{rv.pd.compopen.power.diff}\par{\scriptsize\cellnote{[\num{rv.pd.compopen.power.difflo}, \num{rv.pd.compopen.power.diffhi}]}} & \num{rv.pd.compopen.emotion.diff}\par{\scriptsize\cellnote{[\num{rv.pd.compopen.emotion.difflo}, \num{rv.pd.compopen.emotion.diffhi}]}} & \num{rv.pd.compopen.politeness.diff}\par{\scriptsize\cellnote{[\num{rv.pd.compopen.politeness.difflo}, \num{rv.pd.compopen.politeness.diffhi}]}} \\
\addlinespace[2.5pt]
\msw{comptwo}Qwen3.6-27B, verbal & \num{rv.pd.comptwo.doneneutral.diff}\par{\scriptsize\cellnote{[\num{rv.pd.comptwo.doneneutral.difflo}, \num{rv.pd.comptwo.doneneutral.diffhi}]}} & \best{\num{rv.pd.comptwo.dtwo.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.comptwo.dtwo.difflo}, \num{rv.pd.comptwo.dtwo.diffhi}]}} & \num{rv.pd.comptwo.toxicity.diff}\par{\scriptsize\cellnote{[\num{rv.pd.comptwo.toxicity.difflo}, \num{rv.pd.comptwo.toxicity.diffhi}]}} & \num{rv.pd.comptwo.power.diff}\par{\scriptsize\cellnote{[\num{rv.pd.comptwo.power.difflo}, \num{rv.pd.comptwo.power.diffhi}]}} & \best{\num{rv.pd.comptwo.emotion.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.comptwo.emotion.difflo}, \num{rv.pd.comptwo.emotion.diffhi}]}} & \num{rv.pd.comptwo.politeness.diff}\par{\scriptsize\cellnote{[\num{rv.pd.comptwo.politeness.difflo}, \num{rv.pd.comptwo.politeness.diffhi}]}} \\
\msw{comptwoll}Qwen3.6-27B, likelihood & \num{rv.pd.comptwoll.doneneutral.diff}\par{\scriptsize\cellnote{[\num{rv.pd.comptwoll.doneneutral.difflo}, \num{rv.pd.comptwoll.doneneutral.diffhi}]}} & \num{rv.pd.comptwoll.dtwo.diff}\par{\scriptsize\cellnote{[\num{rv.pd.comptwoll.dtwo.difflo}, \num{rv.pd.comptwoll.dtwo.diffhi}]}} & \num{rv.pd.comptwoll.toxicity.diff}\par{\scriptsize\cellnote{[\num{rv.pd.comptwoll.toxicity.difflo}, \num{rv.pd.comptwoll.toxicity.diffhi}]}} & \num{rv.pd.comptwoll.power.diff}\par{\scriptsize\cellnote{[\num{rv.pd.comptwoll.power.difflo}, \num{rv.pd.comptwoll.power.diffhi}]}} & \num{rv.pd.comptwoll.emotion.diff}\par{\scriptsize\cellnote{[\num{rv.pd.comptwoll.emotion.difflo}, \num{rv.pd.comptwoll.emotion.diffhi}]}} & \num{rv.pd.comptwoll.politeness.diff}\par{\scriptsize\cellnote{[\num{rv.pd.comptwoll.politeness.difflo}, \num{rv.pd.comptwoll.politeness.diffhi}]}} \\
\msw{comptwothink}Qwen3.6-27B, thinking & \num{rv.pd.comptwothink.doneneutral.diff}\par{\scriptsize\cellnote{[\num{rv.pd.comptwothink.doneneutral.difflo}, \num{rv.pd.comptwothink.doneneutral.diffhi}]}} & \num{rv.pd.comptwothink.dtwo.diff}\par{\scriptsize\cellnote{[\num{rv.pd.comptwothink.dtwo.difflo}, \num{rv.pd.comptwothink.dtwo.diffhi}]}} & \num{rv.pd.comptwothink.toxicity.diff}\par{\scriptsize\cellnote{[\num{rv.pd.comptwothink.toxicity.difflo}, \num{rv.pd.comptwothink.toxicity.diffhi}]}} & \num{rv.pd.comptwothink.power.diff}\par{\scriptsize\cellnote{[\num{rv.pd.comptwothink.power.difflo}, \num{rv.pd.comptwothink.power.diffhi}]}} & \num{rv.pd.comptwothink.emotion.diff}\par{\scriptsize\cellnote{[\num{rv.pd.comptwothink.emotion.difflo}, \num{rv.pd.comptwothink.emotion.diffhi}]}} & \num{rv.pd.comptwothink.politeness.diff}\par{\scriptsize\cellnote{[\num{rv.pd.comptwothink.politeness.difflo}, \num{rv.pd.comptwothink.politeness.diffhi}]}} \\
\addlinespace[2.5pt]
\msw{compgem}Gemma-4-31B, verbal & \num{rv.pd.compgem.doneneutral.diff}\par{\scriptsize\cellnote{[\num{rv.pd.compgem.doneneutral.difflo}, \num{rv.pd.compgem.doneneutral.diffhi}]}} & \best{\num{rv.pd.compgem.dtwo.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.compgem.dtwo.difflo}, \num{rv.pd.compgem.dtwo.diffhi}]}} & \num{rv.pd.compgem.toxicity.diff}\par{\scriptsize\cellnote{[\num{rv.pd.compgem.toxicity.difflo}, \num{rv.pd.compgem.toxicity.diffhi}]}} & \num{rv.pd.compgem.power.diff}\par{\scriptsize\cellnote{[\num{rv.pd.compgem.power.difflo}, \num{rv.pd.compgem.power.diffhi}]}} & \num{rv.pd.compgem.emotion.diff}\par{\scriptsize\cellnote{[\num{rv.pd.compgem.emotion.difflo}, \num{rv.pd.compgem.emotion.diffhi}]}} & \num{rv.pd.compgem.politeness.diff}\par{\scriptsize\cellnote{[\num{rv.pd.compgem.politeness.difflo}, \num{rv.pd.compgem.politeness.diffhi}]}} \\
\msw{compgemll}Gemma-4-31B, likelihood & \num{rv.pd.compgemll.doneneutral.diff}\par{\scriptsize\cellnote{[\num{rv.pd.compgemll.doneneutral.difflo}, \num{rv.pd.compgemll.doneneutral.diffhi}]}} & \best{\num{rv.pd.compgemll.dtwo.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.compgemll.dtwo.difflo}, \num{rv.pd.compgemll.dtwo.diffhi}]}} & \num{rv.pd.compgemll.toxicity.diff}\par{\scriptsize\cellnote{[\num{rv.pd.compgemll.toxicity.difflo}, \num{rv.pd.compgemll.toxicity.diffhi}]}} & \num{rv.pd.compgemll.power.diff}\par{\scriptsize\cellnote{[\num{rv.pd.compgemll.power.difflo}, \num{rv.pd.compgemll.power.diffhi}]}} & \num{rv.pd.compgemll.emotion.diff}\par{\scriptsize\cellnote{[\num{rv.pd.compgemll.emotion.difflo}, \num{rv.pd.compgemll.emotion.diffhi}]}} & \num{rv.pd.compgemll.politeness.diff}\par{\scriptsize\cellnote{[\num{rv.pd.compgemll.politeness.difflo}, \num{rv.pd.compgemll.politeness.diffhi}]}} \\*
\addlinespace[2.5pt]
\msw{compmis}Mistral-Small-24B, verbal & \best{\num{rv.pd.compmis.doneneutral.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.compmis.doneneutral.difflo}, \num{rv.pd.compmis.doneneutral.diffhi}]}} & \best{\num{rv.pd.compmis.dtwo.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.compmis.dtwo.difflo}, \num{rv.pd.compmis.dtwo.diffhi}]}} & \num{rv.pd.compmis.toxicity.diff}\par{\scriptsize\cellnote{[\num{rv.pd.compmis.toxicity.difflo}, \num{rv.pd.compmis.toxicity.diffhi}]}} & \num{rv.pd.compmis.power.diff}\par{\scriptsize\cellnote{[\num{rv.pd.compmis.power.difflo}, \num{rv.pd.compmis.power.diffhi}]}} & \best{\num{rv.pd.compmis.emotion.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.compmis.emotion.difflo}, \num{rv.pd.compmis.emotion.diffhi}]}} & \num{rv.pd.compmis.politeness.diff}\par{\scriptsize\cellnote{[\num{rv.pd.compmis.politeness.difflo}, \num{rv.pd.compmis.politeness.diffhi}]}} \\*
\msw{compmisll}Mistral-Small-24B, likelihood & \best{\num{rv.pd.compmisll.doneneutral.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.compmisll.doneneutral.difflo}, \num{rv.pd.compmisll.doneneutral.diffhi}]}} & \best{\num{rv.pd.compmisll.dtwo.diff}}\par{\scriptsize\cellnote{[\num{rv.pd.compmisll.dtwo.difflo}, \num{rv.pd.compmisll.dtwo.diffhi}]}} & \num{rv.pd.compmisll.toxicity.diff}\par{\scriptsize\cellnote{[\num{rv.pd.compmisll.toxicity.difflo}, \num{rv.pd.compmisll.toxicity.diffhi}]}} & \num{rv.pd.compmisll.power.diff}\par{\scriptsize\cellnote{[\num{rv.pd.compmisll.power.difflo}, \num{rv.pd.compmisll.power.diffhi}]}} & \num{rv.pd.compmisll.emotion.diff}\par{\scriptsize\cellnote{[\num{rv.pd.compmisll.emotion.difflo}, \num{rv.pd.compmisll.emotion.diffhi}]}} & \num{rv.pd.compmisll.politeness.diff}\par{\scriptsize\cellnote{[\num{rv.pd.compmisll.politeness.difflo}, \num{rv.pd.compmisll.politeness.diffhi}]}} \\*
\bottomrule
\end{tabular}
\tablenote{Each cell is the accuracy of the model minus that of Jev 1.13.0 on identical decisions in percentage points, with its paired cluster bootstrap interval at \num{p.boot.level} percent over \num{p.boot.pairedreps} replicates beneath. Bold marks a difference that is significant after Holm correction across the models of each dataset at the five percent level.}


==> tables/t12_manifest.tex <==
% Generated by shared/src/t01_tables.py. Do not edit by hand.
% Every numeric cell is a num-macro from numbers.tex; -- means that
% model has no result for this cell yet. Needs paper4a_tables.sty.
\tablestylewide
\begin{tabular}{P{0.1750}P{0.2750}P{0.1050}N{0.0600}P{0.1050}P{0.2800}}
\toprule
\headrow \hd{Model} & \hd{Repository or service} & \hd{Revision} & \hd{Temp.} & \hd{Run date} & \hd{Runtime} \\
\midrule
\tabhead
\groupspan{six}{Hosted}
\msw{jev}Jev 1.13.0 & TypeSafe API, model \texttt{jev-1.13.0} & -- & -- & \texttt{2026-09-24} to\par \texttt{2026-09-30} & hosted service through \texttt{typesafe\_sdk} \\
\groupspan{six}{Open, encoder head}
\msw{layaen}Laya (English) & \texttt{convaiinnovations/laya} & \texttt{55cf4c4ebb} & \num{m.laya.temp} & \texttt{2026-09-24} to\par \texttt{2026-09-29} & \texttt{laya~0.3.20}, \texttt{torch~2.8.0} \\
\msw{layaml}Laya (multilingual) & \texttt{convaiinnovations/laya}, subfolder \texttt{multilingual} & \texttt{55cf4c4ebb} & \num{m.laya.temp} & \texttt{2026-09-24} to\par \texttt{2026-09-29} & \texttt{laya~0.3.20}, \texttt{torch~2.8.0} \\
\groupspan{six}{Open, decoder head}
\msw{kevsmall}Kev-0.8B & \texttt{jaredpalmer/kev-0.8b} & \texttt{9a45d25eb2} & \num{m.kev08b.temp} & \texttt{2026-09-24} to\par \texttt{2026-09-29} & \texttt{torch~2.8.0}, \texttt{kev@73504e51f6}, \texttt{transformers>=5.17} \\
\msw{kevlarge}Kev-9B & \texttt{jaredpalmer/kev-9b} & \texttt{2629c06a5a} & \num{m.kev9b.temp} & \texttt{2026-09-24} to\par \texttt{2026-09-29} & \texttt{torch~2.8.0}, \texttt{kev@73504e51f6}, \texttt{transformers>=5.17} \\
\msw{decider}decider-2b & \texttt{Mapika/decider-2b} & \texttt{d61c1c1608} & \num{m.decider.temp} & \texttt{2026-09-24} to\par \texttt{2026-09-29} & \texttt{torch~2.8.0}, \texttt{kev@73504e51f6}, \texttt{transformers>=5.17} \\
\msw{thisthat}this-that-model-1.0 & \texttt{flock-io/this-that-model-1.0} & \texttt{3d927195c4} & \num{m.thisthat.temp} & \texttt{2026-09-24} to\par \texttt{2026-09-29} & \texttt{torch~2.8.0}, \texttt{kev@73504e51f6}, \texttt{transformers>=5.17}, \texttt{thisthat@542d445efa} \\
\msw{nimble}Nimble-9B & \texttt{bespokelabs/Bespoke-Nimble-9B} & \texttt{bd792f44ec} & \num{m.nimble.temp} & \texttt{2026-09-24} to\par \texttt{2026-09-29} & \texttt{torch~2.8.0}, \texttt{transformers~5.17.0} \\
\groupspan{six}{Generative comparators}
\msw{compopen}Qwen3-14B, verbal & \texttt{Qwen/Qwen3-14B-AWQ} & \texttt{31c69efc29} & \num{m.comparator.temp} & \texttt{2026-09-25} to\par \texttt{2026-09-29} & \texttt{vllm~0.30.0}, \texttt{torch~2.13.0} \\
\msw{comptwo}Qwen3.6-27B, both readouts & \texttt{Qwen/Qwen3.6-27B-FP8} & \texttt{e89b16ebf1} & \num{m.comparator.temp}, \num{m.likelihood.temp} & \texttt{2026-09-27} to\par \texttt{2026-10-01} & \texttt{vllm~0.30.0} \\
\msw{comptwothink}Qwen3.6-27B, thinking & \texttt{Qwen/Qwen3.6-27B-FP8} & \texttt{e89b16ebf1} & \num{m.think.temp} & \texttt{2026-09-30} to\par \texttt{2026-10-01} & \texttt{vllm~0.30.0} \\
\msw{compgem}Gemma-4-31B, both readouts & \texttt{google/gemma-4-31B-it} & \texttt{842da3794e} & \num{m.comparator.temp}, \num{m.likelihood.temp} & \texttt{2026-09-30} & \texttt{vllm~0.30.0}, bf16, eager \\
\msw{compmis}Mistral-Small-24B, both readouts & \texttt{mistralai/Mistral-Small-24B-\allowbreak Instruct-2501} & \texttt{9527884be6} & \num{m.comparator.temp}, \num{m.likelihood.temp} & \texttt{2026-09-30} & \texttt{vllm~0.30.0}, bf16, eager \\
\groupspan{six}{Untuned backbones}
Qwen3.5-0.8B-Base & \texttt{Qwen/Qwen3.5-0.8B-Base} & \texttt{dc7cdfe2ee} & \num{m.likelihood.temp} & \texttt{2026-09-26} to\par \texttt{2026-09-29} & \texttt{torch~2.8.0}, \texttt{transformers~5.17.0} \\
Qwen3.5-2B-Base & \texttt{Qwen/Qwen3.5-2B-Base} & \texttt{b1485b2fa6} & \num{m.likelihood.temp} & \texttt{2026-09-27} to\par \texttt{2026-09-29} & \texttt{torch~2.8.0}, \texttt{transformers~5.17.0} \\*
Qwen3.5-9B-Base & \texttt{Qwen/Qwen3.5-9B-Base} & \texttt{68c46c4b34} & \num{m.likelihood.temp} & \texttt{2026-09-27} to\par \texttt{2026-09-29} & \texttt{torch~2.8.0}, \texttt{transformers~5.17.0} \\*
Qwen3.5-9B & \texttt{Qwen/Qwen3.5-9B} & \texttt{c202236235} & \num{m.likelihood.temp} & \texttt{2026-09-27} to\par \texttt{2026-09-29} & \texttt{torch~2.8.0}, \texttt{transformers~5.17.0} \\*
\bottomrule
\end{tabular}
\tablenote{Revision is the start of the resolved commit of the weights and Temp.\ the served temperature that every answer record reports. The hosted service reports neither, and each response named the pinned model. Laya applies a temperature per question type and option count and records one as its nominal value. The comparators decode greedily or read key likelihoods at a temperature of one, except the thinking mode, which samples its reasoning at the temperature shown with a fixed seed. Qwen3.6-27B, Gemma-4-31B and Mistral-Small-24B ran on a Colab A100 GPU and every other open model on a Colab L4 GPU, and a pin written as a lower bound was resolved at install time.}


==> tables/t14_baselines.tex <==
% Conventional classifier baselines (shared/src/b01_baselines.py), with the hosted
% decision model as reference. Every numeric cell is a num-macro from numbers.tex.
% Needs paper4a_tables.sty.
\tablestylewide
\begin{tabular}{P{0.2400}P{0.1500}N{0.0800}N{0.0750}N{0.0800}N{0.0750}N{0.0750}N{0.0700}N{0.0750}N{0.0550}}
\toprule
\headrow \hdtop{} & \hdtop{} & \hdgroup{two}{D1 typed-decisions} & \hdgroup{five}{D2 CLINC-150} & \hdtop{} \\
\bandrules{3-4,5-9}
\headrow \hdsub{Model} & \hdsub{Training data} & \hdsub{Acc.} & \hdsub{Soft} & \hdsub{Acc.} & \hdsub{ECE ship.} & \hdsub{ECE scal.} & \hdsub{Cov.} & \hdsub{AUROC} & \hdsub{ms} \\
\midrule
\tabhead
\groupspan{ten}{Hosted decision model}
\msw{jev}Jev 1.13.0 & none & \num{e1.jev.doneneutral.acc} & \num{e1.jev.doneneutral.softacc} & \num{e1.jev.dtwo.acc} & \num{e1.jev.dtwo.ece} & \num{rv.ts.jev.dtwo.ecescaled} & \num{e1.jev.dtwo.covfive} & \num{e1.jev.oos.auroc} & \num{e5.jev.d2k150.pfifty} \\
\groupspan{ten}{Supervised classifiers trained on the task}
BERT-base, fine-tuned & CLINC train & -- & -- & \num{bl.bertbaseclinc.d2k150.acc} & \num{bl.bertbaseclinc.d2k150.eceshipped} & \num{bl.bertbaseclinc.d2k150.ecescaled} & \num{bl.bertbaseclinc.d2k150.cov5} & \num{bl.bertbaseclinc.d2k150.aurocoos} & \num{bl.bertbaseclinc.d2k150.latencymsp50gpu} \\
BGE-small embeddings with logistic regression & CLINC train & -- & -- & \num{bl.bgesmalllrclinc.d2k150.acc} & \textbf{\num{bl.bgesmalllrclinc.d2k150.eceshipped}} & \textbf{\num{bl.bgesmalllrclinc.d2k150.ecescaled}} & \num{bl.bgesmalllrclinc.d2k150.cov5} & \num{bl.bgesmalllrclinc.d2k150.aurocoos} & \num{bl.bgesmalllrclinc.d2k150.latencymsp50gpu} \\
BGE-small embeddings with soft-label regression & typed-decisions train & \num{bl.bgesmalllrd1.d1neutral.acc} & \num{bl.bgesmalllrd1.d1neutral.softacc} & -- & -- & -- & -- & -- & \num{bl.bgesmalllrd1.d1neutral.latencymsp50gpu} \\
DeBERTa-v3-large, fine-tuned & typed-decisions train & \textbf{\num{bl.debertalarged1.d1neutral.acc}} & \textbf{\num{bl.debertalarged1.d1neutral.softacc}} & -- & -- & -- & -- & -- & \num{bl.debertalarged1.d1neutral.latencymsp50l4} \\
DeBERTa-v3-large, fine-tuned & CLINC train & -- & -- & \textbf{\num{bl.debertalargeclinc.d2k150.acc}} & \num{bl.debertalargeclinc.d2k150.eceshipped} & \num{bl.debertalargeclinc.d2k150.ecescaled} & \textbf{\num{bl.debertalargeclinc.d2k150.cov5}} & \textbf{\num{bl.debertalargeclinc.d2k150.aurocoos}} & \num{bl.debertalargeclinc.d2k150.latencymsp50l4} \\
\groupspan{ten}{Zero-shot entailment classifier}
DeBERTa-v3-base NLI & none & \num{bl.nlidebertav3base.d1neutral.acc} & \num{bl.nlidebertav3base.d1neutral.softacc} & \num{bl.nlidebertav3base.d2k150.acc} & \num{bl.nlidebertav3base.d2k150.eceshipped} & \num{bl.nlidebertav3base.d2k150.ecescaled} & \num{bl.nlidebertav3base.d2k150.cov5} & \num{bl.nlidebertav3base.d2k150.aurocoos} & \num{bl.nlidebertav3base.d2k150.latencymsp50gpu} \\
\bottomrule
\end{tabular}
\tablenote{Acc.\ is accuracy, Soft the teacher probability of the chosen option, and ECE ship.\ and scal.\ the calibration error as shipped and after one temperature fitted on held-out data. Cov.\ is the in-sample coverage at \num{p.riskfive} percent risk, AUROC the separation of out-of-scope from in-scope requests by the top probability, and ms the median latency per request on CLINC-150, or per typed-decisions state for the regression baseline. The DeBERTa-v3-large classifiers ran on a Colab L4 GPU, the other baselines on a local workstation GPU and the hosted model through its API, so their latencies are not comparable across platforms. Bold marks the best value in each accuracy, calibration, coverage and separation column.}


==> tables/t16_scores.tex <==
% Generated by shared/src/t01_tables.py. Do not edit by hand.
% Every numeric cell is a num-macro from numbers.tex; -- means that
% model has no result for this cell yet. Needs paper4a_tables.sty.
\tablestyle
\setlength{\tabcolsep}{2pt}
\begin{tabular}{P{0.2850}N{0.0596}N{0.0596}N{0.0596}N{0.0596}N{0.0596}N{0.0596}N{0.0596}N{0.0596}N{0.0596}N{0.0596}N{0.0596}N{0.0596}}
\toprule
\headrow \hdtop{} & \hdgroup{two}{D1} & \hdgroup{two}{D2} & \hdgroup{two}{Derail.} & \hdgroup{two}{Power} & \hdgroup{two}{Emo.} & \hdgroup{two}{Pol.} \\
\bandrules{2-3,4-5,6-7,8-9,10-11,12-13}
\headrow \hdsub{Model} & \hdsub{Brier} & \hdsub{NLL} & \hdsub{Brier} & \hdsub{NLL} & \hdsub{Brier} & \hdsub{NLL} & \hdsub{Brier} & \hdsub{NLL} & \hdsub{Brier} & \hdsub{NLL} & \hdsub{Brier} & \hdsub{NLL} \\
\midrule
\tabhead
\groupspan{thirteen}{Hosted}
\msw{jev}Jev 1.13.0 & \num{e1.jev.doneneutral.brier} & \num{e1.jev.doneneutral.nll} & \num{e1.jev.dtwo.brier} & \num{e1.jev.dtwo.nll} & \num{e1.jev.toxicity.brier} & \num{e1.jev.toxicity.nll} & \num{e1.jev.power.brier} & \num{e1.jev.power.nll} & \num{e1.jev.emotion.brier} & \num{e1.jev.emotion.nll} & \num{e1.jev.politeness.brier} & \num{e1.jev.politeness.nll} \\
\groupspan{thirteen}{Open, encoder head}
\msw{layaen}Laya (English) & \num{e1.layaen.doneneutral.brier} & \num{e1.layaen.doneneutral.nll} & -- & -- & \best{\num{e1.layaen.toxicity.brier}} & \best{\num{e1.layaen.toxicity.nll}} & \num{e1.layaen.power.brier} & \best{\num{e1.layaen.power.nll}} & \num{e1.layaen.emotion.brier} & \num{e1.layaen.emotion.nll} & \num{e1.layaen.politeness.brier} & \num{e1.layaen.politeness.nll} \\
\msw{layaml}Laya (multilingual) & \num{e1.layaml.doneneutral.brier} & \num{e1.layaml.doneneutral.nll} & \num{e1.layaml.dtwo.brier} & \num{e1.layaml.dtwo.nll} & \num{e1.layaml.toxicity.brier} & \num{e1.layaml.toxicity.nll} & \num{e1.layaml.power.brier} & \num{e1.layaml.power.nll} & \num{e1.layaml.emotion.brier} & \num{e1.layaml.emotion.nll} & \num{e1.layaml.politeness.brier} & \num{e1.layaml.politeness.nll} \\
\groupspan{thirteen}{Open, decoder head}
\msw{kevsmall}Kev-0.8B & \num{e1.kevsmall.doneneutral.brier} & \num{e1.kevsmall.doneneutral.nll} & \num{e1.kevsmall.dtwo.brier} & \num{e1.kevsmall.dtwo.nll} & \num{e1.kevsmall.toxicity.brier} & \num{e1.kevsmall.toxicity.nll} & \num{e1.kevsmall.power.brier} & \num{e1.kevsmall.power.nll} & \num{e1.kevsmall.emotion.brier} & \num{e1.kevsmall.emotion.nll} & \num{e1.kevsmall.politeness.brier} & \num{e1.kevsmall.politeness.nll} \\
\msw{kevlarge}Kev-9B & \num{e1.kevlarge.doneneutral.brier} & \num{e1.kevlarge.doneneutral.nll} & \num{e1.kevlarge.dtwo.brier} & \num{e1.kevlarge.dtwo.nll} & \num{e1.kevlarge.toxicity.brier} & \num{e1.kevlarge.toxicity.nll} & \best{\num{e1.kevlarge.power.brier}} & \num{e1.kevlarge.power.nll} & \num{e1.kevlarge.emotion.brier} & \num{e1.kevlarge.emotion.nll} & \num{e1.kevlarge.politeness.brier} & \num{e1.kevlarge.politeness.nll} \\
\msw{decider}decider-2b & \num{e1.decider.doneneutral.brier} & \num{e1.decider.doneneutral.nll} & \num{e1.decider.dtwo.brier} & \num{e1.decider.dtwo.nll} & \num{e1.decider.toxicity.brier} & \num{e1.decider.toxicity.nll} & \num{e1.decider.power.brier} & \num{e1.decider.power.nll} & \best{\num{e1.decider.emotion.brier}} & \best{\num{e1.decider.emotion.nll}} & \num{e1.decider.politeness.brier} & \num{e1.decider.politeness.nll} \\
\msw{thisthat}this-that-model-1.0 & \num{e1.thisthat.doneneutral.brier} & \num{e1.thisthat.doneneutral.nll} & \num{e1.thisthat.dtwo.brier} & \num{e1.thisthat.dtwo.nll} & \num{e1.thisthat.toxicity.brier} & \num{e1.thisthat.toxicity.nll} & \num{e1.thisthat.power.brier} & \num{e1.thisthat.power.nll} & \num{e1.thisthat.emotion.brier} & \num{e1.thisthat.emotion.nll} & \num{e1.thisthat.politeness.brier} & \num{e1.thisthat.politeness.nll} \\
\msw{nimble}Nimble-9B & \num{e1.nimble.doneneutral.brier} & \num{e1.nimble.doneneutral.nll} & \num{e1.nimble.dtwo.brier} & \num{e1.nimble.dtwo.nll} & \num{e1.nimble.toxicity.brier} & \num{e1.nimble.toxicity.nll} & \num{e1.nimble.power.brier} & \num{e1.nimble.power.nll} & \num{e1.nimble.emotion.brier} & \num{e1.nimble.emotion.nll} & \num{e1.nimble.politeness.brier} & \num{e1.nimble.politeness.nll} \\
\groupspan{thirteen}{Generative comparators}
\msw{compopen}Qwen3-14B, verbal & \num{e1.compopen.doneneutral.brier} & \num{e1.compopen.doneneutral.nll} & \num{e1.compopen.dtwo.brier} & \num{e1.compopen.dtwo.nll} & \num{e1.compopen.toxicity.brier} & \num{e1.compopen.toxicity.nll} & \num{e1.compopen.power.brier} & \num{e1.compopen.power.nll} & \num{e1.compopen.emotion.brier} & \num{e1.compopen.emotion.nll} & \num{e1.compopen.politeness.brier} & \num{e1.compopen.politeness.nll} \\
\addlinespace[2.5pt]
\msw{comptwo}Qwen3.6-27B, verbal & \num{e1.comptwo.doneneutral.brier} & \num{e1.comptwo.doneneutral.nll} & \num{e1.comptwo.dtwo.brier} & \num{e1.comptwo.dtwo.nll} & \num{e1.comptwo.toxicity.brier} & \num{e1.comptwo.toxicity.nll} & \num{e1.comptwo.power.brier} & \num{e1.comptwo.power.nll} & \num{e1.comptwo.emotion.brier} & \num{e1.comptwo.emotion.nll} & \num{e1.comptwo.politeness.brier} & \num{e1.comptwo.politeness.nll} \\
\msw{comptwoll}Qwen3.6-27B, likelihood & \best{\num{e1.comptwoll.doneneutral.brier}} & \best{\num{e1.comptwoll.doneneutral.nll}} & \num{e1.comptwoll.dtwo.brier} & \num{e1.comptwoll.dtwo.nll} & \num{e1.comptwoll.toxicity.brier} & \num{e1.comptwoll.toxicity.nll} & \num{e1.comptwoll.power.brier} & \num{e1.comptwoll.power.nll} & \num{e1.comptwoll.emotion.brier} & \num{e1.comptwoll.emotion.nll} & \num{e1.comptwoll.politeness.brier} & \num{e1.comptwoll.politeness.nll} \\
\msw{comptwothink}Qwen3.6-27B, thinking & \num{e1.comptwothink.doneneutral.brier} & \num{e1.comptwothink.doneneutral.nll} & \num{e1.comptwothink.dtwo.brier} & \num{e1.comptwothink.dtwo.nll} & \num{e1.comptwothink.toxicity.brier} & \num{e1.comptwothink.toxicity.nll} & \num{e1.comptwothink.power.brier} & \num{e1.comptwothink.power.nll} & \num{e1.comptwothink.emotion.brier} & \num{e1.comptwothink.emotion.nll} & \num{e1.comptwothink.politeness.brier} & \num{e1.comptwothink.politeness.nll} \\
\addlinespace[2.5pt]
\msw{compgem}Gemma-4-31B, verbal & \num{e1.compgem.doneneutral.brier} & \num{e1.compgem.doneneutral.nll} & \best{\num{e1.compgem.dtwo.brier}} & \best{\num{e1.compgem.dtwo.nll}} & \num{e1.compgem.toxicity.brier} & \num{e1.compgem.toxicity.nll} & \num{e1.compgem.power.brier} & \num{e1.compgem.power.nll} & \num{e1.compgem.emotion.brier} & \num{e1.compgem.emotion.nll} & \num{e1.compgem.politeness.brier} & \num{e1.compgem.politeness.nll} \\
\msw{compgemll}Gemma-4-31B, likelihood & \num{e1.compgemll.doneneutral.brier} & \num{e1.compgemll.doneneutral.nll} & \num{e1.compgemll.dtwo.brier} & \num{e1.compgemll.dtwo.nll} & \num{e1.compgemll.toxicity.brier} & \num{e1.compgemll.toxicity.nll} & \num{e1.compgemll.power.brier} & \num{e1.compgemll.power.nll} & \num{e1.compgemll.emotion.brier} & \num{e1.compgemll.emotion.nll} & \num{e1.compgemll.politeness.brier} & \num{e1.compgemll.politeness.nll} \\*
\addlinespace[2.5pt]
\msw{compmis}Mistral-Small-24B, verbal & \num{e1.compmis.doneneutral.brier} & \num{e1.compmis.doneneutral.nll} & \num{e1.compmis.dtwo.brier} & \num{e1.compmis.dtwo.nll} & \num{e1.compmis.toxicity.brier} & \num{e1.compmis.toxicity.nll} & \num{e1.compmis.power.brier} & \num{e1.compmis.power.nll} & \num{e1.compmis.emotion.brier} & \num{e1.compmis.emotion.nll} & \num{e1.compmis.politeness.brier} & \num{e1.compmis.politeness.nll} \\*
\msw{compmisll}Mistral-Small-24B, likelihood & \num{e1.compmisll.doneneutral.brier} & \num{e1.compmisll.doneneutral.nll} & \num{e1.compmisll.dtwo.brier} & \num{e1.compmisll.dtwo.nll} & \num{e1.compmisll.toxicity.brier} & \num{e1.compmisll.toxicity.nll} & \num{e1.compmisll.power.brier} & \num{e1.compmisll.power.nll} & \num{e1.compmisll.emotion.brier} & \num{e1.compmisll.emotion.nll} & \best{\num{e1.compmisll.politeness.brier}} & \best{\num{e1.compmisll.politeness.nll}} \\*
\bottomrule
\end{tabular}
\tablenote{Brier is the multi-class Brier score and NLL the negative log-likelihood of the reference label, both from the probabilities as shipped. Bold marks the lowest value in each column, with ties bolded, and the over-budget Laya (multilingual) cells on D2 are shown but not ranked.}


==> tables/t17_backbones.tex <==
% Generated by shared/src/t01_tables.py. Do not edit by hand.
% Every numeric cell is a num-macro from numbers.tex; -- means that
% model has no result for this cell yet. Needs paper4a_tables.sty.
\tablestylewide
\begin{tabular}{P{0.1500}P{0.1600}N{0.1150}N{0.1150}N{0.1150}N{0.1150}N{0.1150}N{0.1150}}
\toprule
\headrow \hdtop{} & \hdtop{} & \hdgroup{six}{Accuracy difference} \\
\bandrules{3-8}
\headrow \hdsub{Decision model} & \hdsub{Untuned backbone} & \hdsub{D1} & \hdsub{D2} & \hdsub{Derail.} & \hdsub{Power} & \hdsub{Emotion} & \hdsub{Polite.} \\
\midrule
\tabhead
\msw{kevsmall}Kev-0.8B & Qwen3.5-0.8B-Base & \num{bb.kevsmall.bbsmallbase.doneneutral.acc.diff}\par{\scriptsize\cellnote{[\num{bb.kevsmall.bbsmallbase.doneneutral.acc.lo}, \num{bb.kevsmall.bbsmallbase.doneneutral.acc.hi}]}} & \best{\num{bb.kevsmall.bbsmallbase.dtwo.acc.diff}}\par{\scriptsize\cellnote{[\num{bb.kevsmall.bbsmallbase.dtwo.acc.lo}, \num{bb.kevsmall.bbsmallbase.dtwo.acc.hi}]}} & \num{bb.kevsmall.bbsmallbase.toxicity.acc.diff}\par{\scriptsize\cellnote{[\num{bb.kevsmall.bbsmallbase.toxicity.acc.lo}, \num{bb.kevsmall.bbsmallbase.toxicity.acc.hi}]}} & \num{bb.kevsmall.bbsmallbase.power.acc.diff}\par{\scriptsize\cellnote{[\num{bb.kevsmall.bbsmallbase.power.acc.lo}, \num{bb.kevsmall.bbsmallbase.power.acc.hi}]}} & \best{\num{bb.kevsmall.bbsmallbase.emotion.acc.diff}}\par{\scriptsize\cellnote{[\num{bb.kevsmall.bbsmallbase.emotion.acc.lo}, \num{bb.kevsmall.bbsmallbase.emotion.acc.hi}]}} & \best{\num{bb.kevsmall.bbsmallbase.politeness.acc.diff}}\par{\scriptsize\cellnote{[\num{bb.kevsmall.bbsmallbase.politeness.acc.lo}, \num{bb.kevsmall.bbsmallbase.politeness.acc.hi}]}} \\
\msw{kevlarge}Kev-9B & Qwen3.5-9B-Base & \best{\num{bb.kevlarge.bbninebase.doneneutral.acc.diff}}\par{\scriptsize\cellnote{[\num{bb.kevlarge.bbninebase.doneneutral.acc.lo}, \num{bb.kevlarge.bbninebase.doneneutral.acc.hi}]}} & \best{\num{bb.kevlarge.bbninebase.dtwo.acc.diff}}\par{\scriptsize\cellnote{[\num{bb.kevlarge.bbninebase.dtwo.acc.lo}, \num{bb.kevlarge.bbninebase.dtwo.acc.hi}]}} & \num{bb.kevlarge.bbninebase.toxicity.acc.diff}\par{\scriptsize\cellnote{[\num{bb.kevlarge.bbninebase.toxicity.acc.lo}, \num{bb.kevlarge.bbninebase.toxicity.acc.hi}]}} & \num{bb.kevlarge.bbninebase.power.acc.diff}\par{\scriptsize\cellnote{[\num{bb.kevlarge.bbninebase.power.acc.lo}, \num{bb.kevlarge.bbninebase.power.acc.hi}]}} & \best{\num{bb.kevlarge.bbninebase.emotion.acc.diff}}\par{\scriptsize\cellnote{[\num{bb.kevlarge.bbninebase.emotion.acc.lo}, \num{bb.kevlarge.bbninebase.emotion.acc.hi}]}} & \num{bb.kevlarge.bbninebase.politeness.acc.diff}\par{\scriptsize\cellnote{[\num{bb.kevlarge.bbninebase.politeness.acc.lo}, \num{bb.kevlarge.bbninebase.politeness.acc.hi}]}} \\
\msw{nimble}Nimble-9B & Qwen3.5-9B & \best{\num{bb.nimble.bbnine.doneneutral.acc.diff}}\par{\scriptsize\cellnote{[\num{bb.nimble.bbnine.doneneutral.acc.lo}, \num{bb.nimble.bbnine.doneneutral.acc.hi}]}} & \best{\num{bb.nimble.bbnine.dtwo.acc.diff}}\par{\scriptsize\cellnote{[\num{bb.nimble.bbnine.dtwo.acc.lo}, \num{bb.nimble.bbnine.dtwo.acc.hi}]}} & \num{bb.nimble.bbnine.toxicity.acc.diff}\par{\scriptsize\cellnote{[\num{bb.nimble.bbnine.toxicity.acc.lo}, \num{bb.nimble.bbnine.toxicity.acc.hi}]}} & \num{bb.nimble.bbnine.power.acc.diff}\par{\scriptsize\cellnote{[\num{bb.nimble.bbnine.power.acc.lo}, \num{bb.nimble.bbnine.power.acc.hi}]}} & \num{bb.nimble.bbnine.emotion.acc.diff}\par{\scriptsize\cellnote{[\num{bb.nimble.bbnine.emotion.acc.lo}, \num{bb.nimble.bbnine.emotion.acc.hi}]}} & \num{bb.nimble.bbnine.politeness.acc.diff}\par{\scriptsize\cellnote{[\num{bb.nimble.bbnine.politeness.acc.lo}, \num{bb.nimble.bbnine.politeness.acc.hi}]}} \\*
\msw{decider}decider-2b & Qwen3.5-2B-Base & \best{\num{bb.decider.bbtwobase.doneneutral.acc.diff}}\par{\scriptsize\cellnote{[\num{bb.decider.bbtwobase.doneneutral.acc.lo}, \num{bb.decider.bbtwobase.doneneutral.acc.hi}]}} & \best{\num{bb.decider.bbtwobase.dtwo.acc.diff}}\par{\scriptsize\cellnote{[\num{bb.decider.bbtwobase.dtwo.acc.lo}, \num{bb.decider.bbtwobase.dtwo.acc.hi}]}} & \num{bb.decider.bbtwobase.toxicity.acc.diff}\par{\scriptsize\cellnote{[\num{bb.decider.bbtwobase.toxicity.acc.lo}, \num{bb.decider.bbtwobase.toxicity.acc.hi}]}} & \num{bb.decider.bbtwobase.power.acc.diff}\par{\scriptsize\cellnote{[\num{bb.decider.bbtwobase.power.acc.lo}, \num{bb.decider.bbtwobase.power.acc.hi}]}} & \best{\num{bb.decider.bbtwobase.emotion.acc.diff}}\par{\scriptsize\cellnote{[\num{bb.decider.bbtwobase.emotion.acc.lo}, \num{bb.decider.bbtwobase.emotion.acc.hi}]}} & \num{bb.decider.bbtwobase.politeness.acc.diff}\par{\scriptsize\cellnote{[\num{bb.decider.bbtwobase.politeness.acc.lo}, \num{bb.decider.bbtwobase.politeness.acc.hi}]}} \\*
\msw{thisthat}this-that-model-1.0 & Qwen3.5-2B-Base & \best{\num{bb.thisthat.bbtwobase.doneneutral.acc.diff}}\par{\scriptsize\cellnote{[\num{bb.thisthat.bbtwobase.doneneutral.acc.lo}, \num{bb.thisthat.bbtwobase.doneneutral.acc.hi}]}} & \best{\num{bb.thisthat.bbtwobase.dtwo.acc.diff}}\par{\scriptsize\cellnote{[\num{bb.thisthat.bbtwobase.dtwo.acc.lo}, \num{bb.thisthat.bbtwobase.dtwo.acc.hi}]}} & \num{bb.thisthat.bbtwobase.toxicity.acc.diff}\par{\scriptsize\cellnote{[\num{bb.thisthat.bbtwobase.toxicity.acc.lo}, \num{bb.thisthat.bbtwobase.toxicity.acc.hi}]}} & \num{bb.thisthat.bbtwobase.power.acc.diff}\par{\scriptsize\cellnote{[\num{bb.thisthat.bbtwobase.power.acc.lo}, \num{bb.thisthat.bbtwobase.power.acc.hi}]}} & \best{\num{bb.thisthat.bbtwobase.emotion.acc.diff}}\par{\scriptsize\cellnote{[\num{bb.thisthat.bbtwobase.emotion.acc.lo}, \num{bb.thisthat.bbtwobase.emotion.acc.hi}]}} & \num{bb.thisthat.bbtwobase.politeness.acc.diff}\par{\scriptsize\cellnote{[\num{bb.thisthat.bbtwobase.politeness.acc.lo}, \num{bb.thisthat.bbtwobase.politeness.acc.hi}]}} \\*
\bottomrule
\end{tabular}
\par\vspace{6pt}
\begin{tabular}{P{0.1500}P{0.1600}N{0.1150}N{0.1150}N{0.1150}N{0.1150}N{0.1150}N{0.1150}}
\toprule
\headrow \hdtop{} & \hdtop{} & \hdgroup{six}{Calibration error difference} \\
\bandrules{3-8}
\headrow \hdsub{Decision model} & \hdsub{Untuned backbone} & \hdsub{D1} & \hdsub{D2} & \hdsub{Derail.} & \hdsub{Power} & \hdsub{Emotion} & \hdsub{Polite.} \\
\midrule
\tabhead
\msw{kevsmall}Kev-0.8B & Qwen3.5-0.8B-Base & \best{\num{bb.kevsmall.bbsmallbase.doneneutral.ece.diff}}\par{\scriptsize\cellnote{[\num{bb.kevsmall.bbsmallbase.doneneutral.ece.lo}, \num{bb.kevsmall.bbsmallbase.doneneutral.ece.hi}]}} & \best{\num{bb.kevsmall.bbsmallbase.dtwo.ece.diff}}\par{\scriptsize\cellnote{[\num{bb.kevsmall.bbsmallbase.dtwo.ece.lo}, \num{bb.kevsmall.bbsmallbase.dtwo.ece.hi}]}} & \best{\num{bb.kevsmall.bbsmallbase.toxicity.ece.diff}}\par{\scriptsize\cellnote{[\num{bb.kevsmall.bbsmallbase.toxicity.ece.lo}, \num{bb.kevsmall.bbsmallbase.toxicity.ece.hi}]}} & \num{bb.kevsmall.bbsmallbase.power.ece.diff}\par{\scriptsize\cellnote{[\num{bb.kevsmall.bbsmallbase.power.ece.lo}, \num{bb.kevsmall.bbsmallbase.power.ece.hi}]}} & \best{\num{bb.kevsmall.bbsmallbase.emotion.ece.diff}}\par{\scriptsize\cellnote{[\num{bb.kevsmall.bbsmallbase.emotion.ece.lo}, \num{bb.kevsmall.bbsmallbase.emotion.ece.hi}]}} & \best{\num{bb.kevsmall.bbsmallbase.politeness.ece.diff}}\par{\scriptsize\cellnote{[\num{bb.kevsmall.bbsmallbase.politeness.ece.lo}, \num{bb.kevsmall.bbsmallbase.politeness.ece.hi}]}} \\
\msw{kevlarge}Kev-9B & Qwen3.5-9B-Base & \best{\num{bb.kevlarge.bbninebase.doneneutral.ece.diff}}\par{\scriptsize\cellnote{[\num{bb.kevlarge.bbninebase.doneneutral.ece.lo}, \num{bb.kevlarge.bbninebase.doneneutral.ece.hi}]}} & \best{\num{bb.kevlarge.bbninebase.dtwo.ece.diff}}\par{\scriptsize\cellnote{[\num{bb.kevlarge.bbninebase.dtwo.ece.lo}, \num{bb.kevlarge.bbninebase.dtwo.ece.hi}]}} & \best{\num{bb.kevlarge.bbninebase.toxicity.ece.diff}}\par{\scriptsize\cellnote{[\num{bb.kevlarge.bbninebase.toxicity.ece.lo}, \num{bb.kevlarge.bbninebase.toxicity.ece.hi}]}} & \best{\num{bb.kevlarge.bbninebase.power.ece.diff}}\par{\scriptsize\cellnote{[\num{bb.kevlarge.bbninebase.power.ece.lo}, \num{bb.kevlarge.bbninebase.power.ece.hi}]}} & \best{\num{bb.kevlarge.bbninebase.emotion.ece.diff}}\par{\scriptsize\cellnote{[\num{bb.kevlarge.bbninebase.emotion.ece.lo}, \num{bb.kevlarge.bbninebase.emotion.ece.hi}]}} & \num{bb.kevlarge.bbninebase.politeness.ece.diff}\par{\scriptsize\cellnote{[\num{bb.kevlarge.bbninebase.politeness.ece.lo}, \num{bb.kevlarge.bbninebase.politeness.ece.hi}]}} \\
\msw{nimble}Nimble-9B & Qwen3.5-9B & \best{\num{bb.nimble.bbnine.doneneutral.ece.diff}}\par{\scriptsize\cellnote{[\num{bb.nimble.bbnine.doneneutral.ece.lo}, \num{bb.nimble.bbnine.doneneutral.ece.hi}]}} & \num{bb.nimble.bbnine.dtwo.ece.diff}\par{\scriptsize\cellnote{[\num{bb.nimble.bbnine.dtwo.ece.lo}, \num{bb.nimble.bbnine.dtwo.ece.hi}]}} & \best{\num{bb.nimble.bbnine.toxicity.ece.diff}}\par{\scriptsize\cellnote{[\num{bb.nimble.bbnine.toxicity.ece.lo}, \num{bb.nimble.bbnine.toxicity.ece.hi}]}} & \best{\num{bb.nimble.bbnine.power.ece.diff}}\par{\scriptsize\cellnote{[\num{bb.nimble.bbnine.power.ece.lo}, \num{bb.nimble.bbnine.power.ece.hi}]}} & \best{\num{bb.nimble.bbnine.emotion.ece.diff}}\par{\scriptsize\cellnote{[\num{bb.nimble.bbnine.emotion.ece.lo}, \num{bb.nimble.bbnine.emotion.ece.hi}]}} & \best{\num{bb.nimble.bbnine.politeness.ece.diff}}\par{\scriptsize\cellnote{[\num{bb.nimble.bbnine.politeness.ece.lo}, \num{bb.nimble.bbnine.politeness.ece.hi}]}} \\*
\msw{decider}decider-2b & Qwen3.5-2B-Base & \best{\num{bb.decider.bbtwobase.doneneutral.ece.diff}}\par{\scriptsize\cellnote{[\num{bb.decider.bbtwobase.doneneutral.ece.lo}, \num{bb.decider.bbtwobase.doneneutral.ece.hi}]}} & \best{\num{bb.decider.bbtwobase.dtwo.ece.diff}}\par{\scriptsize\cellnote{[\num{bb.decider.bbtwobase.dtwo.ece.lo}, \num{bb.decider.bbtwobase.dtwo.ece.hi}]}} & \best{\num{bb.decider.bbtwobase.toxicity.ece.diff}}\par{\scriptsize\cellnote{[\num{bb.decider.bbtwobase.toxicity.ece.lo}, \num{bb.decider.bbtwobase.toxicity.ece.hi}]}} & \best{\num{bb.decider.bbtwobase.power.ece.diff}}\par{\scriptsize\cellnote{[\num{bb.decider.bbtwobase.power.ece.lo}, \num{bb.decider.bbtwobase.power.ece.hi}]}} & \best{\num{bb.decider.bbtwobase.emotion.ece.diff}}\par{\scriptsize\cellnote{[\num{bb.decider.bbtwobase.emotion.ece.lo}, \num{bb.decider.bbtwobase.emotion.ece.hi}]}} & \best{\num{bb.decider.bbtwobase.politeness.ece.diff}}\par{\scriptsize\cellnote{[\num{bb.decider.bbtwobase.politeness.ece.lo}, \num{bb.decider.bbtwobase.politeness.ece.hi}]}} \\*
\msw{thisthat}this-that-model-1.0 & Qwen3.5-2B-Base & \best{\num{bb.thisthat.bbtwobase.doneneutral.ece.diff}}\par{\scriptsize\cellnote{[\num{bb.thisthat.bbtwobase.doneneutral.ece.lo}, \num{bb.thisthat.bbtwobase.doneneutral.ece.hi}]}} & \best{\num{bb.thisthat.bbtwobase.dtwo.ece.diff}}\par{\scriptsize\cellnote{[\num{bb.thisthat.bbtwobase.dtwo.ece.lo}, \num{bb.thisthat.bbtwobase.dtwo.ece.hi}]}} & \best{\num{bb.thisthat.bbtwobase.toxicity.ece.diff}}\par{\scriptsize\cellnote{[\num{bb.thisthat.bbtwobase.toxicity.ece.lo}, \num{bb.thisthat.bbtwobase.toxicity.ece.hi}]}} & \best{\num{bb.thisthat.bbtwobase.power.ece.diff}}\par{\scriptsize\cellnote{[\num{bb.thisthat.bbtwobase.power.ece.lo}, \num{bb.thisthat.bbtwobase.power.ece.hi}]}} & \num{bb.thisthat.bbtwobase.emotion.ece.diff}\par{\scriptsize\cellnote{[\num{bb.thisthat.bbtwobase.emotion.ece.lo}, \num{bb.thisthat.bbtwobase.emotion.ece.hi}]}} & \best{\num{bb.thisthat.bbtwobase.politeness.ece.diff}}\par{\scriptsize\cellnote{[\num{bb.thisthat.bbtwobase.politeness.ece.lo}, \num{bb.thisthat.bbtwobase.politeness.ece.hi}]}} \\*
\bottomrule
\end{tabular}
\par\vspace{6pt}
\begin{tabular}{P{0.1500}P{0.1600}N{0.1150}N{0.1150}N{0.1150}N{0.1150}N{0.1150}N{0.1150}}
\toprule
\headrow \hdtop{} & \hdtop{} & \hdgroup{six}{Flip difference under option names} \\
\bandrules{3-8}
\headrow \hdsub{Decision model} & \hdsub{Untuned backbone} & \hdsub{D1 swap} & \hdsub{D1 digits} & \hdsub{D1 rand.} & \hdsub{Derail. swap} & \hdsub{Derail. rand.} & \hdsub{Power swap} \\
\midrule
\tabhead
\msw{kevsmall}Kev-0.8B & Qwen3.5-0.8B-Base & \num{bb.kevsmall.bbsmallbase.donekswap.flips.diff}\par{\scriptsize\cellnote{[\num{bb.kevsmall.bbsmallbase.donekswap.flips.lo}, \num{bb.kevsmall.bbsmallbase.donekswap.flips.hi}]}} & \best{\num{bb.kevsmall.bbsmallbase.donek01.flips.diff}}\par{\scriptsize\cellnote{[\num{bb.kevsmall.bbsmallbase.donek01.flips.lo}, \num{bb.kevsmall.bbsmallbase.donek01.flips.hi}]}} & \best{\num{bb.kevsmall.bbsmallbase.donekrand.flips.diff}}\par{\scriptsize\cellnote{[\num{bb.kevsmall.bbsmallbase.donekrand.flips.lo}, \num{bb.kevsmall.bbsmallbase.donekrand.flips.hi}]}} & \best{\num{bb.kevsmall.bbsmallbase.toxicitykswap.flips.diff}}\par{\scriptsize\cellnote{[\num{bb.kevsmall.bbsmallbase.toxicitykswap.flips.lo}, \num{bb.kevsmall.bbsmallbase.toxicitykswap.flips.hi}]}} & \best{\num{bb.kevsmall.bbsmallbase.toxicitykrand.flips.diff}}\par{\scriptsize\cellnote{[\num{bb.kevsmall.bbsmallbase.toxicitykrand.flips.lo}, \num{bb.kevsmall.bbsmallbase.toxicitykrand.flips.hi}]}} & \best{\num{bb.kevsmall.bbsmallbase.powerkswap.flips.diff}}\par{\scriptsize\cellnote{[\num{bb.kevsmall.bbsmallbase.powerkswap.flips.lo}, \num{bb.kevsmall.bbsmallbase.powerkswap.flips.hi}]}} \\
\msw{kevlarge}Kev-9B & Qwen3.5-9B-Base & \best{\num{bb.kevlarge.bbninebase.donekswap.flips.diff}}\par{\scriptsize\cellnote{[\num{bb.kevlarge.bbninebase.donekswap.flips.lo}, \num{bb.kevlarge.bbninebase.donekswap.flips.hi}]}} & \num{bb.kevlarge.bbninebase.donek01.flips.diff}\par{\scriptsize\cellnote{[\num{bb.kevlarge.bbninebase.donek01.flips.lo}, \num{bb.kevlarge.bbninebase.donek01.flips.hi}]}} & \best{\num{bb.kevlarge.bbninebase.donekrand.flips.diff}}\par{\scriptsize\cellnote{[\num{bb.kevlarge.bbninebase.donekrand.flips.lo}, \num{bb.kevlarge.bbninebase.donekrand.flips.hi}]}} & \best{\num{bb.kevlarge.bbninebase.toxicitykswap.flips.diff}}\par{\scriptsize\cellnote{[\num{bb.kevlarge.bbninebase.toxicitykswap.flips.lo}, \num{bb.kevlarge.bbninebase.toxicitykswap.flips.hi}]}} & \best{\num{bb.kevlarge.bbninebase.toxicitykrand.flips.diff}}\par{\scriptsize\cellnote{[\num{bb.kevlarge.bbninebase.toxicitykrand.flips.lo}, \num{bb.kevlarge.bbninebase.toxicitykrand.flips.hi}]}} & \best{\num{bb.kevlarge.bbninebase.powerkswap.flips.diff}}\par{\scriptsize\cellnote{[\num{bb.kevlarge.bbninebase.powerkswap.flips.lo}, \num{bb.kevlarge.bbninebase.powerkswap.flips.hi}]}} \\
\msw{nimble}Nimble-9B & Qwen3.5-9B & \best{\num{bb.nimble.bbnine.donekswap.flips.diff}}\par{\scriptsize\cellnote{[\num{bb.nimble.bbnine.donekswap.flips.lo}, \num{bb.nimble.bbnine.donekswap.flips.hi}]}} & \best{\num{bb.nimble.bbnine.donek01.flips.diff}}\par{\scriptsize\cellnote{[\num{bb.nimble.bbnine.donek01.flips.lo}, \num{bb.nimble.bbnine.donek01.flips.hi}]}} & \best{\num{bb.nimble.bbnine.donekrand.flips.diff}}\par{\scriptsize\cellnote{[\num{bb.nimble.bbnine.donekrand.flips.lo}, \num{bb.nimble.bbnine.donekrand.flips.hi}]}} & \best{\num{bb.nimble.bbnine.toxicitykswap.flips.diff}}\par{\scriptsize\cellnote{[\num{bb.nimble.bbnine.toxicitykswap.flips.lo}, \num{bb.nimble.bbnine.toxicitykswap.flips.hi}]}} & \best{\num{bb.nimble.bbnine.toxicitykrand.flips.diff}}\par{\scriptsize\cellnote{[\num{bb.nimble.bbnine.toxicitykrand.flips.lo}, \num{bb.nimble.bbnine.toxicitykrand.flips.hi}]}} & \best{\num{bb.nimble.bbnine.powerkswap.flips.diff}}\par{\scriptsize\cellnote{[\num{bb.nimble.bbnine.powerkswap.flips.lo}, \num{bb.nimble.bbnine.powerkswap.flips.hi}]}} \\*
\msw{decider}decider-2b & Qwen3.5-2B-Base & \num{bb.decider.bbtwobase.donekswap.flips.diff}\par{\scriptsize\cellnote{[\num{bb.decider.bbtwobase.donekswap.flips.lo}, \num{bb.decider.bbtwobase.donekswap.flips.hi}]}} & \num{bb.decider.bbtwobase.donek01.flips.diff}\par{\scriptsize\cellnote{[\num{bb.decider.bbtwobase.donek01.flips.lo}, \num{bb.decider.bbtwobase.donek01.flips.hi}]}} & \num{bb.decider.bbtwobase.donekrand.flips.diff}\par{\scriptsize\cellnote{[\num{bb.decider.bbtwobase.donekrand.flips.lo}, \num{bb.decider.bbtwobase.donekrand.flips.hi}]}} & \best{\num{bb.decider.bbtwobase.toxicitykswap.flips.diff}}\par{\scriptsize\cellnote{[\num{bb.decider.bbtwobase.toxicitykswap.flips.lo}, \num{bb.decider.bbtwobase.toxicitykswap.flips.hi}]}} & \best{\num{bb.decider.bbtwobase.toxicitykrand.flips.diff}}\par{\scriptsize\cellnote{[\num{bb.decider.bbtwobase.toxicitykrand.flips.lo}, \num{bb.decider.bbtwobase.toxicitykrand.flips.hi}]}} & \best{\num{bb.decider.bbtwobase.powerkswap.flips.diff}}\par{\scriptsize\cellnote{[\num{bb.decider.bbtwobase.powerkswap.flips.lo}, \num{bb.decider.bbtwobase.powerkswap.flips.hi}]}} \\*
\msw{thisthat}this-that-model-1.0 & Qwen3.5-2B-Base & \num{bb.thisthat.bbtwobase.donekswap.flips.diff}\par{\scriptsize\cellnote{[\num{bb.thisthat.bbtwobase.donekswap.flips.lo}, \num{bb.thisthat.bbtwobase.donekswap.flips.hi}]}} & \num{bb.thisthat.bbtwobase.donek01.flips.diff}\par{\scriptsize\cellnote{[\num{bb.thisthat.bbtwobase.donek01.flips.lo}, \num{bb.thisthat.bbtwobase.donek01.flips.hi}]}} & \num{bb.thisthat.bbtwobase.donekrand.flips.diff}\par{\scriptsize\cellnote{[\num{bb.thisthat.bbtwobase.donekrand.flips.lo}, \num{bb.thisthat.bbtwobase.donekrand.flips.hi}]}} & \best{\num{bb.thisthat.bbtwobase.toxicitykswap.flips.diff}}\par{\scriptsize\cellnote{[\num{bb.thisthat.bbtwobase.toxicitykswap.flips.lo}, \num{bb.thisthat.bbtwobase.toxicitykswap.flips.hi}]}} & \best{\num{bb.thisthat.bbtwobase.toxicitykrand.flips.diff}}\par{\scriptsize\cellnote{[\num{bb.thisthat.bbtwobase.toxicitykrand.flips.lo}, \num{bb.thisthat.bbtwobase.toxicitykrand.flips.hi}]}} & \best{\num{bb.thisthat.bbtwobase.powerkswap.flips.diff}}\par{\scriptsize\cellnote{[\num{bb.thisthat.bbtwobase.powerkswap.flips.lo}, \num{bb.thisthat.bbtwobase.powerkswap.flips.hi}]}} \\*
\bottomrule
\end{tabular}
\tablenote{Each cell is the decision model minus the untuned backbone it adapts on identical decisions, in points of accuracy or of shipped top-label calibration error, or in flips per hundred decisions against the aligned names, with its paired cluster bootstrap interval beneath. The backbones are scored by the likelihood of each option key after a plain prompt. The decider-2b and this-that-model-1.0 checkpoints were trained on CLINC-150, and this-that-model-1.0 is adapted from decider-2b. Bold marks a difference significant after Holm correction across the five pairs of its column at the five percent level.}


==> tables/t18_oos_option.tex <==
% Generated by shared/src/t01_tables.py. Do not edit by hand.
% Every numeric cell is a num-macro from numbers.tex; -- means that
% model has no result for this cell yet. Needs paper4a_tables.sty.
\tablestyle
\begin{tabular}{P{0.2850}N{0.1192}N{0.1192}N{0.1192}N{0.1192}N{0.1192}N{0.1192}}
\toprule
\headrow \hdtop{} & \hdgroup{three}{Answers with the option} & \hdgroup{three}{Gate at the in-scope risk target} \\
\bandrules{2-4,5-7}
\headrow \hdsub{Model} & \hdsub{In-scope acc.} & \hdsub{OOS chosen} & \hdsub{In-scope lost} & \hdsub{Answered} & \hdsub{Accepted} & \hdsub{Without option} \\
\midrule
\tabhead
\groupspan{seven}{Hosted}
\msw{jev}Jev 1.13.0 & \num{oo.jev.accin} & \num{oo.jev.oosrecall} & \num{oo.jev.falsereject} & \num{oo.jev.gcov}\par{\scriptsize\cellnote{[\num{oo.jev.gcovlo}, \num{oo.jev.gcovhi}]}} & \num{oo.jev.gfar}\par{\scriptsize\cellnote{[\num{oo.jev.gfarlo}, \num{oo.jev.gfarhi}]}} & \num{rv.gate.jev.far} \\
\groupspan{seven}{Open, encoder head}
\msw{layaml}Laya (multilingual) & \num{oo.layaml.accin} & \num{oo.layaml.oosrecall} & \num{oo.layaml.falsereject} & \num{oo.layaml.gcov}\par{\scriptsize\cellnote{[\num{oo.layaml.gcovlo}, \num{oo.layaml.gcovhi}]}} & \num{oo.layaml.gfar}\par{\scriptsize\cellnote{[\num{oo.layaml.gfarlo}, \num{oo.layaml.gfarhi}]}} & \num{rv.gate.layaml.far} \\
\groupspan{seven}{Open, decoder head}
\msw{kevsmall}Kev-0.8B & \num{oo.kevsmall.accin} & \num{oo.kevsmall.oosrecall} & \num{oo.kevsmall.falsereject} & \num{oo.kevsmall.gcov}\par{\scriptsize\cellnote{[\num{oo.kevsmall.gcovlo}, \num{oo.kevsmall.gcovhi}]}} & \num{oo.kevsmall.gfar}\par{\scriptsize\cellnote{[\num{oo.kevsmall.gfarlo}, \num{oo.kevsmall.gfarhi}]}} & \num{rv.gate.kevsmall.far} \\
\msw{kevlarge}Kev-9B & \num{oo.kevlarge.accin} & \num{oo.kevlarge.oosrecall} & \num{oo.kevlarge.falsereject} & \num{oo.kevlarge.gcov}\par{\scriptsize\cellnote{[\num{oo.kevlarge.gcovlo}, \num{oo.kevlarge.gcovhi}]}} & \best{\num{oo.kevlarge.gfar}}\par{\scriptsize\cellnote{[\num{oo.kevlarge.gfarlo}, \num{oo.kevlarge.gfarhi}]}} & \num{rv.gate.kevlarge.far} \\
\msw{decider}decider-2b & \num{oo.decider.accin} & \num{oo.decider.oosrecall} & \num{oo.decider.falsereject} & \num{oo.decider.gcov}\par{\scriptsize\cellnote{[\num{oo.decider.gcovlo}, \num{oo.decider.gcovhi}]}} & \num{oo.decider.gfar}\par{\scriptsize\cellnote{[\num{oo.decider.gfarlo}, \num{oo.decider.gfarhi}]}} & \num{rv.gate.decider.far} \\
\msw{thisthat}this-that-model-1.0 & \num{oo.thisthat.accin} & \num{oo.thisthat.oosrecall} & \num{oo.thisthat.falsereject} & \num{oo.thisthat.gcov}\par{\scriptsize\cellnote{[\num{oo.thisthat.gcovlo}, \num{oo.thisthat.gcovhi}]}} & \num{oo.thisthat.gfar}\par{\scriptsize\cellnote{[\num{oo.thisthat.gfarlo}, \num{oo.thisthat.gfarhi}]}} & \num{rv.gate.thisthat.far} \\
\msw{nimble}Nimble-9B & \num{oo.nimble.accin} & \num{oo.nimble.oosrecall} & \num{oo.nimble.falsereject} & \num{oo.nimble.gcov}\par{\scriptsize\cellnote{[\num{oo.nimble.gcovlo}, \num{oo.nimble.gcovhi}]}} & \num{oo.nimble.gfar}\par{\scriptsize\cellnote{[\num{oo.nimble.gfarlo}, \num{oo.nimble.gfarhi}]}} & \num{rv.gate.nimble.far} \\
\groupspan{seven}{Generative comparators}
\msw{compopen}Qwen3-14B, verbal & \num{oo.compopen.accin} & \num{oo.compopen.oosrecall} & \num{oo.compopen.falsereject} & \num{oo.compopen.gcov}\par{\scriptsize\cellnote{[\num{oo.compopen.gcovlo}, \num{oo.compopen.gcovhi}]}} & \num{oo.compopen.gfar}\par{\scriptsize\cellnote{[\num{oo.compopen.gfarlo}, \num{oo.compopen.gfarhi}]}} & \num{rv.gate.compopen.far} \\
\addlinespace[2.5pt]
\msw{comptwo}Qwen3.6-27B, verbal & \num{oo.comptwo.accin} & \num{oo.comptwo.oosrecall} & \num{oo.comptwo.falsereject} & \num{oo.comptwo.gcov}\par{\scriptsize\cellnote{[\num{oo.comptwo.gcovlo}, \num{oo.comptwo.gcovhi}]}} & \num{oo.comptwo.gfar}\par{\scriptsize\cellnote{[\num{oo.comptwo.gfarlo}, \num{oo.comptwo.gfarhi}]}} & \num{rv.gate.comptwo.far} \\
\msw{comptwoll}Qwen3.6-27B, likelihood & \num{oo.comptwoll.accin} & \num{oo.comptwoll.oosrecall} & \num{oo.comptwoll.falsereject} & \num{oo.comptwoll.gcov}\par{\scriptsize\cellnote{[\num{oo.comptwoll.gcovlo}, \num{oo.comptwoll.gcovhi}]}} & \num{oo.comptwoll.gfar}\par{\scriptsize\cellnote{[\num{oo.comptwoll.gfarlo}, \num{oo.comptwoll.gfarhi}]}} & \num{rv.gate.comptwoll.far} \\
\msw{comptwothink}Qwen3.6-27B, thinking & \num{oo.comptwothink.accin} & \num{oo.comptwothink.oosrecall} & \num{oo.comptwothink.falsereject} & \num{oo.comptwothink.gcov}\par{\scriptsize\cellnote{[\num{oo.comptwothink.gcovlo}, \num{oo.comptwothink.gcovhi}]}} & \num{oo.comptwothink.gfar}\par{\scriptsize\cellnote{[\num{oo.comptwothink.gfarlo}, \num{oo.comptwothink.gfarhi}]}} & \num{rv.gate.comptwothink.far} \\
\addlinespace[2.5pt]
\msw{compgem}Gemma-4-31B, verbal & \num{oo.compgem.accin} & \num{oo.compgem.oosrecall} & \num{oo.compgem.falsereject} & \num{oo.compgem.gcov}\par{\scriptsize\cellnote{[\num{oo.compgem.gcovlo}, \num{oo.compgem.gcovhi}]}} & \num{oo.compgem.gfar}\par{\scriptsize\cellnote{[\num{oo.compgem.gfarlo}, \num{oo.compgem.gfarhi}]}} & \num{rv.gate.compgem.far} \\
\msw{compgemll}Gemma-4-31B, likelihood & \num{oo.compgemll.accin} & \num{oo.compgemll.oosrecall} & \num{oo.compgemll.falsereject} & \num{oo.compgemll.gcov}\par{\scriptsize\cellnote{[\num{oo.compgemll.gcovlo}, \num{oo.compgemll.gcovhi}]}} & \num{oo.compgemll.gfar}\par{\scriptsize\cellnote{[\num{oo.compgemll.gfarlo}, \num{oo.compgemll.gfarhi}]}} & \num{rv.gate.compgemll.far} \\*
\addlinespace[2.5pt]
\msw{compmis}Mistral-Small-24B, verbal & \num{oo.compmis.accin} & \num{oo.compmis.oosrecall} & \num{oo.compmis.falsereject} & \num{oo.compmis.gcov}\par{\scriptsize\cellnote{[\num{oo.compmis.gcovlo}, \num{oo.compmis.gcovhi}]}} & \num{oo.compmis.gfar}\par{\scriptsize\cellnote{[\num{oo.compmis.gfarlo}, \num{oo.compmis.gfarhi}]}} & \num{rv.gate.compmis.far} \\*
\msw{compmisll}Mistral-Small-24B, likelihood & \num{oo.compmisll.accin} & \num{oo.compmisll.oosrecall} & \num{oo.compmisll.falsereject} & \num{oo.compmisll.gcov}\par{\scriptsize\cellnote{[\num{oo.compmisll.gcovlo}, \num{oo.compmisll.gcovhi}]}} & \num{oo.compmisll.gfar}\par{\scriptsize\cellnote{[\num{oo.compmisll.gfarlo}, \num{oo.compmisll.gfarhi}]}} & \num{rv.gate.compmisll.far} \\*
\bottomrule
\end{tabular}
\tablenote{The \num{n.d2k150.requests} CLINC-150 requests are asked with the \num{p.kall} intents and one further option named out of scope. In-scope acc.\ counts an in-scope request answered with that option as an error, OOS chosen is the share of out-of-scope requests answered with that option and In-scope lost the share of in-scope requests answered with it. The gate routes a request when it is not answered with the option and its top probability reaches a held-out threshold that targets \num{p.riskfive} percent in-scope risk. Answered is its in-scope coverage and Accepted its out-of-scope false acceptance, beside the false acceptance of the same gate without the option, with cluster bootstrap intervals beneath Answered and Accepted. Laya (English) refused every request with this option set and is not listed. Bold marks the lowest false acceptance among models that answer at least half of the in-scope requests.}


==> tables/t20_readouts.tex <==
% Generated by shared/src/t01_tables.py. Do not edit by hand.
% Every numeric cell is a num-macro from numbers.tex; -- means that
% model has no result for this cell yet. Needs paper4a_tables.sty.
\tablestyle
\begin{tabular}{P{0.2850}P{0.2150}N{0.1000}N{0.1000}N{0.1000}N{0.1000}N{0.1000}}
\toprule
\headrow \hd{Model} & \hd{Measure} & \hd{D1} & \hd{D2} & \hd{Emotion} & \hd{GoEmo.} & \hd{Bank.} \\
\midrule
\tabhead
\groupspan{seven}{Generative comparators}
\msw{compopen}Qwen3-14B, verbal & Unusable share & \num{vr.compopen.doneneutral.failshare} & \num{vr.compopen.dtwo.failshare} & \num{vr.compopen.emotion.failshare} & \num{vr.compopen.goemo.failshare} & \num{vr.compopen.banking.failshare} \\
 & Accuracy, fixed parser & \num{vr.compopen.doneneutral.accstrict} & \num{vr.compopen.dtwo.accstrict} & \num{vr.compopen.emotion.accstrict} & \num{vr.compopen.goemo.accstrict} & \num{vr.compopen.banking.accstrict} \\
 & Accuracy, lenient & \num{vr.compopen.doneneutral.acclenient} & \num{vr.compopen.dtwo.acclenient} & \num{vr.compopen.emotion.acclenient} & \num{vr.compopen.goemo.acclenient} & \num{vr.compopen.banking.acclenient} \\
\addlinespace[2.5pt]
\msw{comptwo}Qwen3.6-27B, verbal & Unusable share & \num{vr.comptwo.doneneutral.failshare} & \num{vr.comptwo.dtwo.failshare} & \num{vr.comptwo.emotion.failshare} & \num{vr.comptwo.goemo.failshare} & \num{vr.comptwo.banking.failshare} \\
 & Accuracy, fixed parser & \num{vr.comptwo.doneneutral.accstrict} & \num{vr.comptwo.dtwo.accstrict} & \num{vr.comptwo.emotion.accstrict} & \num{vr.comptwo.goemo.accstrict} & \num{vr.comptwo.banking.accstrict} \\
 & Accuracy, lenient & \num{vr.comptwo.doneneutral.acclenient} & \num{vr.comptwo.dtwo.acclenient} & \num{vr.comptwo.emotion.acclenient} & \num{vr.comptwo.goemo.acclenient} & \num{vr.comptwo.banking.acclenient} \\
\addlinespace[2.5pt]
\msw{comptwothink}Qwen3.6-27B, thinking & Unusable share & \num{vr.comptwothink.doneneutral.failshare} & \num{vr.comptwothink.dtwo.failshare} & \num{vr.comptwothink.emotion.failshare} & \num{vr.comptwothink.goemo.failshare} & \num{vr.comptwothink.banking.failshare} \\
 & Accuracy, fixed parser & \num{vr.comptwothink.doneneutral.accstrict} & \num{vr.comptwothink.dtwo.accstrict} & \num{vr.comptwothink.emotion.accstrict} & \num{vr.comptwothink.goemo.accstrict} & \num{vr.comptwothink.banking.accstrict} \\
 & Accuracy, lenient & \num{vr.comptwothink.doneneutral.acclenient} & \num{vr.comptwothink.dtwo.acclenient} & \num{vr.comptwothink.emotion.acclenient} & \num{vr.comptwothink.goemo.acclenient} & \num{vr.comptwothink.banking.acclenient} \\
\addlinespace[2.5pt]
\msw{compgem}Gemma-4-31B, verbal & Unusable share & \num{vr.compgem.doneneutral.failshare} & \num{vr.compgem.dtwo.failshare} & \num{vr.compgem.emotion.failshare} & \num{vr.compgem.goemo.failshare} & \num{vr.compgem.banking.failshare} \\
 & Accuracy, fixed parser & \num{vr.compgem.doneneutral.accstrict} & \num{vr.compgem.dtwo.accstrict} & \num{vr.compgem.emotion.accstrict} & \num{vr.compgem.goemo.accstrict} & \num{vr.compgem.banking.accstrict} \\
 & Accuracy, lenient & \num{vr.compgem.doneneutral.acclenient} & \num{vr.compgem.dtwo.acclenient} & \num{vr.compgem.emotion.acclenient} & \num{vr.compgem.goemo.acclenient} & \num{vr.compgem.banking.acclenient} \\
\addlinespace[2.5pt]
\msw{compmis}Mistral-Small-24B, verbal & Unusable share & \num{vr.compmis.doneneutral.failshare} & \num{vr.compmis.dtwo.failshare} & \num{vr.compmis.emotion.failshare} & \num{vr.compmis.goemo.failshare} & \num{vr.compmis.banking.failshare} \\*
 & Accuracy, fixed parser & \num{vr.compmis.doneneutral.accstrict} & \num{vr.compmis.dtwo.accstrict} & \num{vr.compmis.emotion.accstrict} & \num{vr.compmis.goemo.accstrict} & \num{vr.compmis.banking.accstrict} \\*
 & Accuracy, lenient & \num{vr.compmis.doneneutral.acclenient} & \num{vr.compmis.dtwo.acclenient} & \num{vr.compmis.emotion.acclenient} & \num{vr.compmis.goemo.acclenient} & \num{vr.compmis.banking.acclenient} \\*
\bottomrule
\end{tabular}
\tablenote{Unusable share counts decisions whose reply has no parseable JSON after any reasoning, or names an option by its key joined to its description. The fixed parser, used in every other table, scores such a decision as a uniform distribution, and the lenient re-parse accepts a key followed by its description. GoEmo.\ is GoEmotions and Bank.\ is Banking77.}


==> tables/t21_risk_control.tex <==
% Generated by shared/src/t01_tables.py. Do not edit by hand.
% Every numeric cell is a num-macro from numbers.tex; -- means that
% model has no result for this cell yet. Needs paper4a_tables.sty.
\tablestyle
\begin{tabular}{P{0.2850}N{0.1192}N{0.1192}N{0.1192}N{0.1192}N{0.1192}N{0.1192}}
\toprule
\headrow \hdtop{} & \hdgroup{three}{D1 typed-decisions} & \hdgroup{three}{D2 CLINC-150} \\
\bandrules{2-4,5-7}
\headrow \hdsub{Model} & \hdsub{Coverage} & \hdsub{Accepted} & \hdsub{Risk} & \hdsub{Coverage} & \hdsub{Accepted} & \hdsub{Risk} \\
\midrule
\tabhead
\groupspan{seven}{Hosted}
\msw{jev}Jev 1.13.0 & \num{rc.jev.doneneutral.cov} & \num{rc.jev.doneneutral.accepted} & \num{rc.jev.doneneutral.risk} & \best{\num{rc.jev.dtwo.cov}} & \num{rc.jev.dtwo.accepted} & \num{rc.jev.dtwo.risk} \\
\groupspan{seven}{Open, encoder head}
\msw{layaen}Laya (English) & \num{rc.layaen.doneneutral.cov} & \num{rc.layaen.doneneutral.accepted} & -- & -- & -- & -- \\
\msw{layaml}Laya (multilingual) & \num{rc.layaml.doneneutral.cov} & \num{rc.layaml.doneneutral.accepted} & -- & \num{rc.layaml.dtwo.cov} & \num{rc.layaml.dtwo.accepted} & -- \\
\groupspan{seven}{Open, decoder head}
\msw{kevsmall}Kev-0.8B & \num{rc.kevsmall.doneneutral.cov} & \num{rc.kevsmall.doneneutral.accepted} & -- & \num{rc.kevsmall.dtwo.cov} & \num{rc.kevsmall.dtwo.accepted} & -- \\
\msw{kevlarge}Kev-9B & \num{rc.kevlarge.doneneutral.cov} & \num{rc.kevlarge.doneneutral.accepted} & -- & \num{rc.kevlarge.dtwo.cov} & \num{rc.kevlarge.dtwo.accepted} & -- \\
\msw{decider}decider-2b & \num{rc.decider.doneneutral.cov} & \num{rc.decider.doneneutral.accepted} & -- & \num{rc.decider.dtwo.cov} & \num{rc.decider.dtwo.accepted} & \num{rc.decider.dtwo.risk} \\
\msw{thisthat}this-that-model-1.0 & \num{rc.thisthat.doneneutral.cov} & \num{rc.thisthat.doneneutral.accepted} & -- & \num{rc.thisthat.dtwo.cov} & \num{rc.thisthat.dtwo.accepted} & \num{rc.thisthat.dtwo.risk} \\
\msw{nimble}Nimble-9B & \num{rc.nimble.doneneutral.cov} & \num{rc.nimble.doneneutral.accepted} & \num{rc.nimble.doneneutral.risk} & \num{rc.nimble.dtwo.cov} & \num{rc.nimble.dtwo.accepted} & -- \\
\groupspan{seven}{Generative comparators}
\msw{compopen}Qwen3-14B, verbal & \num{rc.compopen.doneneutral.cov} & \num{rc.compopen.doneneutral.accepted} & -- & \num{rc.compopen.dtwo.cov} & \num{rc.compopen.dtwo.accepted} & -- \\
\addlinespace[2.5pt]
\msw{comptwo}Qwen3.6-27B, verbal & \num{rc.comptwo.doneneutral.cov} & \num{rc.comptwo.doneneutral.accepted} & -- & \num{rc.comptwo.dtwo.cov} & \num{rc.comptwo.dtwo.accepted} & -- \\
\msw{comptwoll}Qwen3.6-27B, likelihood & \best{\num{rc.comptwoll.doneneutral.cov}} & \num{rc.comptwoll.doneneutral.accepted} & \num{rc.comptwoll.doneneutral.risk} & \num{rc.comptwoll.dtwo.cov} & \num{rc.comptwoll.dtwo.accepted} & \num{rc.comptwoll.dtwo.risk} \\
\msw{comptwothink}Qwen3.6-27B, thinking & \num{rc.comptwothink.doneneutral.cov} & \num{rc.comptwothink.doneneutral.accepted} & -- & \num{rc.comptwothink.dtwo.cov} & \num{rc.comptwothink.dtwo.accepted} & \num{rc.comptwothink.dtwo.risk} \\
\addlinespace[2.5pt]
\msw{compgem}Gemma-4-31B, verbal & \num{rc.compgem.doneneutral.cov} & \num{rc.compgem.doneneutral.accepted} & -- & \num{rc.compgem.dtwo.cov} & \num{rc.compgem.dtwo.accepted} & \num{rc.compgem.dtwo.risk} \\
\msw{compgemll}Gemma-4-31B, likelihood & \num{rc.compgemll.doneneutral.cov} & \num{rc.compgemll.doneneutral.accepted} & -- & \num{rc.compgemll.dtwo.cov} & \num{rc.compgemll.dtwo.accepted} & -- \\*
\addlinespace[2.5pt]
\msw{compmis}Mistral-Small-24B, verbal & \num{rc.compmis.doneneutral.cov} & \num{rc.compmis.doneneutral.accepted} & -- & \num{rc.compmis.dtwo.cov} & \num{rc.compmis.dtwo.accepted} & -- \\*
\msw{compmisll}Mistral-Small-24B, likelihood & \num{rc.compmisll.doneneutral.cov} & \num{rc.compmisll.doneneutral.accepted} & -- & \num{rc.compmisll.dtwo.cov} & \num{rc.compmisll.dtwo.accepted} & -- \\*
\bottomrule
\end{tabular}
\tablenote{The threshold is the lowest of \num{rc.gridsize} fixed candidates whose accepted decisions on the calibration data pass an exact binomial test of an error rate at or below \num{rc.alpha} percent, with a Bonferroni correction over the candidates at \num{rc.confidence} percent confidence. Coverage and Risk are the accepted share and its error rate on the scored decisions, and Accepted counts those decisions, with a dash where none is accepted. Bold marks the highest coverage on each dataset, with ties bolded.}


==> tables/t22_cascade_qwen.tex <==
% Generated by shared/src/t01_tables.py. Do not edit by hand.
% Every numeric cell is a num-macro from numbers.tex; -- means that
% model has no result for this cell yet. Needs paper4a_tables.sty.
\tablestylewide
\begin{tabular}{P{0.2600}N{0.0850}N{0.0850}N{0.0850}P{0.1300}N{0.0750}P{0.1100}N{0.0850}N{0.0850}}
\toprule
\headrow \hdtop{D1 typed-decisions} & \hdgroup{two}{Single stage} & \hdgroup{four}{Cascade} & \hdgroup{two}{Escalation} \\
\bandrules{2-3,4-7,8-9}
\headrow \hdsub{First stage} & \hdsub{First} & \hdsub{Second} & \hdsub{Accuracy} & \hdsub{} & \hdsub{Gain\mk{}} & \hdsub{} & \hdsub{Esc.} & \hdsub{Cost} \\
\midrule
\tabhead
\groupspan{nine}{Escalation to Qwen3-14B, verbal}
\msw{jev}Jev 1.13.0 & \num{e6.jev.compopen.doneneutral.accfirst} & \num{e6.jev.compopen.doneneutral.accsecond} & \num{rv.cas.jev.compopen.doneneutral.acc} & {\scriptsize\cellnote{[\num{rv.cas.jev.compopen.doneneutral.acclo}, \num{rv.cas.jev.compopen.doneneutral.acchi}]}} & \num{rv.cas.jev.compopen.doneneutral.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.jev.compopen.doneneutral.gainlo}, \num{rv.cas.jev.compopen.doneneutral.gainhi}]}} & \num{rv.cas.jev.compopen.doneneutral.esc} & \num{rv.cas.jev.compopen.doneneutral.costfrac} \\
\msw{layaen}Laya (English) & \num{e6.layaen.compopen.doneneutral.accfirst} & \num{e6.layaen.compopen.doneneutral.accsecond} & \num{rv.cas.layaen.compopen.doneneutral.acc} & {\scriptsize\cellnote{[\num{rv.cas.layaen.compopen.doneneutral.acclo}, \num{rv.cas.layaen.compopen.doneneutral.acchi}]}} & \num{rv.cas.layaen.compopen.doneneutral.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.layaen.compopen.doneneutral.gainlo}, \num{rv.cas.layaen.compopen.doneneutral.gainhi}]}} & \num{rv.cas.layaen.compopen.doneneutral.esc} & \num{rv.cas.layaen.compopen.doneneutral.costfrac} \\
\msw{layaml}Laya (multilingual) & \num{e6.layaml.compopen.doneneutral.accfirst} & \num{e6.layaml.compopen.doneneutral.accsecond} & \num{rv.cas.layaml.compopen.doneneutral.acc} & {\scriptsize\cellnote{[\num{rv.cas.layaml.compopen.doneneutral.acclo}, \num{rv.cas.layaml.compopen.doneneutral.acchi}]}} & \num{rv.cas.layaml.compopen.doneneutral.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.layaml.compopen.doneneutral.gainlo}, \num{rv.cas.layaml.compopen.doneneutral.gainhi}]}} & \num{rv.cas.layaml.compopen.doneneutral.esc} & \num{rv.cas.layaml.compopen.doneneutral.costfrac} \\
\msw{kevsmall}Kev-0.8B & \num{e6.kevsmall.compopen.doneneutral.accfirst} & \num{e6.kevsmall.compopen.doneneutral.accsecond} & \num{rv.cas.kevsmall.compopen.doneneutral.acc} & {\scriptsize\cellnote{[\num{rv.cas.kevsmall.compopen.doneneutral.acclo}, \num{rv.cas.kevsmall.compopen.doneneutral.acchi}]}} & \num{rv.cas.kevsmall.compopen.doneneutral.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.kevsmall.compopen.doneneutral.gainlo}, \num{rv.cas.kevsmall.compopen.doneneutral.gainhi}]}} & \num{rv.cas.kevsmall.compopen.doneneutral.esc} & \num{rv.cas.kevsmall.compopen.doneneutral.costfrac} \\
\msw{kevlarge}Kev-9B & \num{e6.kevlarge.compopen.doneneutral.accfirst} & \num{e6.kevlarge.compopen.doneneutral.accsecond} & \num{rv.cas.kevlarge.compopen.doneneutral.acc} & {\scriptsize\cellnote{[\num{rv.cas.kevlarge.compopen.doneneutral.acclo}, \num{rv.cas.kevlarge.compopen.doneneutral.acchi}]}} & \num{rv.cas.kevlarge.compopen.doneneutral.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.kevlarge.compopen.doneneutral.gainlo}, \num{rv.cas.kevlarge.compopen.doneneutral.gainhi}]}} & \num{rv.cas.kevlarge.compopen.doneneutral.esc} & \num{rv.cas.kevlarge.compopen.doneneutral.costfrac} \\
\msw{decider}decider-2b & \num{e6.decider.compopen.doneneutral.accfirst} & \num{e6.decider.compopen.doneneutral.accsecond} & \num{rv.cas.decider.compopen.doneneutral.acc} & {\scriptsize\cellnote{[\num{rv.cas.decider.compopen.doneneutral.acclo}, \num{rv.cas.decider.compopen.doneneutral.acchi}]}} & \num{rv.cas.decider.compopen.doneneutral.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.decider.compopen.doneneutral.gainlo}, \num{rv.cas.decider.compopen.doneneutral.gainhi}]}} & \num{rv.cas.decider.compopen.doneneutral.esc} & \num{rv.cas.decider.compopen.doneneutral.costfrac} \\
\msw{thisthat}this-that-model-1.0 & \num{e6.thisthat.compopen.doneneutral.accfirst} & \num{e6.thisthat.compopen.doneneutral.accsecond} & \num{rv.cas.thisthat.compopen.doneneutral.acc} & {\scriptsize\cellnote{[\num{rv.cas.thisthat.compopen.doneneutral.acclo}, \num{rv.cas.thisthat.compopen.doneneutral.acchi}]}} & \num{rv.cas.thisthat.compopen.doneneutral.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.thisthat.compopen.doneneutral.gainlo}, \num{rv.cas.thisthat.compopen.doneneutral.gainhi}]}} & \num{rv.cas.thisthat.compopen.doneneutral.esc} & \num{rv.cas.thisthat.compopen.doneneutral.costfrac} \\
\msw{nimble}Nimble-9B & \num{e6.nimble.compopen.doneneutral.accfirst} & \num{e6.nimble.compopen.doneneutral.accsecond} & \num{rv.cas.nimble.compopen.doneneutral.acc} & {\scriptsize\cellnote{[\num{rv.cas.nimble.compopen.doneneutral.acclo}, \num{rv.cas.nimble.compopen.doneneutral.acchi}]}} & \num{rv.cas.nimble.compopen.doneneutral.gain}\mk{\symfull} & {\scriptsize\cellnote{[\num{rv.cas.nimble.compopen.doneneutral.gainlo}, \num{rv.cas.nimble.compopen.doneneutral.gainhi}]}} & \num{rv.cas.nimble.compopen.doneneutral.esc} & \num{rv.cas.nimble.compopen.doneneutral.costfrac} \\
\groupspan{nine}{Escalation to Qwen3.6-27B, verbal}
\msw{jev}Jev 1.13.0 & \num{e6.jev.comptwo.doneneutral.accfirst} & \num{e6.jev.comptwo.doneneutral.accsecond} & \num{rv.cas.jev.comptwo.doneneutral.acc} & {\scriptsize\cellnote{[\num{rv.cas.jev.comptwo.doneneutral.acclo}, \num{rv.cas.jev.comptwo.doneneutral.acchi}]}} & \num{rv.cas.jev.comptwo.doneneutral.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.jev.comptwo.doneneutral.gainlo}, \num{rv.cas.jev.comptwo.doneneutral.gainhi}]}} & \num{rv.cas.jev.comptwo.doneneutral.esc} & \num{rv.cas.jev.comptwo.doneneutral.costfrac} \\
\msw{layaen}Laya (English) & \num{e6.layaen.comptwo.doneneutral.accfirst} & \num{e6.layaen.comptwo.doneneutral.accsecond} & \num{rv.cas.layaen.comptwo.doneneutral.acc} & {\scriptsize\cellnote{[\num{rv.cas.layaen.comptwo.doneneutral.acclo}, \num{rv.cas.layaen.comptwo.doneneutral.acchi}]}} & \num{rv.cas.layaen.comptwo.doneneutral.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.layaen.comptwo.doneneutral.gainlo}, \num{rv.cas.layaen.comptwo.doneneutral.gainhi}]}} & \num{rv.cas.layaen.comptwo.doneneutral.esc} & \num{rv.cas.layaen.comptwo.doneneutral.costfrac} \\
\msw{layaml}Laya (multilingual) & \num{e6.layaml.comptwo.doneneutral.accfirst} & \num{e6.layaml.comptwo.doneneutral.accsecond} & \num{rv.cas.layaml.comptwo.doneneutral.acc} & {\scriptsize\cellnote{[\num{rv.cas.layaml.comptwo.doneneutral.acclo}, \num{rv.cas.layaml.comptwo.doneneutral.acchi}]}} & \num{rv.cas.layaml.comptwo.doneneutral.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.layaml.comptwo.doneneutral.gainlo}, \num{rv.cas.layaml.comptwo.doneneutral.gainhi}]}} & \num{rv.cas.layaml.comptwo.doneneutral.esc} & \num{rv.cas.layaml.comptwo.doneneutral.costfrac} \\
\msw{kevsmall}Kev-0.8B & \num{e6.kevsmall.comptwo.doneneutral.accfirst} & \num{e6.kevsmall.comptwo.doneneutral.accsecond} & \num{rv.cas.kevsmall.comptwo.doneneutral.acc} & {\scriptsize\cellnote{[\num{rv.cas.kevsmall.comptwo.doneneutral.acclo}, \num{rv.cas.kevsmall.comptwo.doneneutral.acchi}]}} & \num{rv.cas.kevsmall.comptwo.doneneutral.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.kevsmall.comptwo.doneneutral.gainlo}, \num{rv.cas.kevsmall.comptwo.doneneutral.gainhi}]}} & \num{rv.cas.kevsmall.comptwo.doneneutral.esc} & \num{rv.cas.kevsmall.comptwo.doneneutral.costfrac} \\
\msw{kevlarge}Kev-9B & \num{e6.kevlarge.comptwo.doneneutral.accfirst} & \num{e6.kevlarge.comptwo.doneneutral.accsecond} & \num{rv.cas.kevlarge.comptwo.doneneutral.acc} & {\scriptsize\cellnote{[\num{rv.cas.kevlarge.comptwo.doneneutral.acclo}, \num{rv.cas.kevlarge.comptwo.doneneutral.acchi}]}} & \num{rv.cas.kevlarge.comptwo.doneneutral.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.kevlarge.comptwo.doneneutral.gainlo}, \num{rv.cas.kevlarge.comptwo.doneneutral.gainhi}]}} & \num{rv.cas.kevlarge.comptwo.doneneutral.esc} & \num{rv.cas.kevlarge.comptwo.doneneutral.costfrac} \\
\msw{decider}decider-2b & \num{e6.decider.comptwo.doneneutral.accfirst} & \num{e6.decider.comptwo.doneneutral.accsecond} & \num{rv.cas.decider.comptwo.doneneutral.acc} & {\scriptsize\cellnote{[\num{rv.cas.decider.comptwo.doneneutral.acclo}, \num{rv.cas.decider.comptwo.doneneutral.acchi}]}} & \num{rv.cas.decider.comptwo.doneneutral.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.decider.comptwo.doneneutral.gainlo}, \num{rv.cas.decider.comptwo.doneneutral.gainhi}]}} & \num{rv.cas.decider.comptwo.doneneutral.esc} & \num{rv.cas.decider.comptwo.doneneutral.costfrac} \\
\msw{thisthat}this-that-model-1.0 & \num{e6.thisthat.comptwo.doneneutral.accfirst} & \num{e6.thisthat.comptwo.doneneutral.accsecond} & \num{rv.cas.thisthat.comptwo.doneneutral.acc} & {\scriptsize\cellnote{[\num{rv.cas.thisthat.comptwo.doneneutral.acclo}, \num{rv.cas.thisthat.comptwo.doneneutral.acchi}]}} & \num{rv.cas.thisthat.comptwo.doneneutral.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.thisthat.comptwo.doneneutral.gainlo}, \num{rv.cas.thisthat.comptwo.doneneutral.gainhi}]}} & \num{rv.cas.thisthat.comptwo.doneneutral.esc} & \num{rv.cas.thisthat.comptwo.doneneutral.costfrac} \\
\msw{nimble}Nimble-9B & \num{e6.nimble.comptwo.doneneutral.accfirst} & \num{e6.nimble.comptwo.doneneutral.accsecond} & \num{rv.cas.nimble.comptwo.doneneutral.acc} & {\scriptsize\cellnote{[\num{rv.cas.nimble.comptwo.doneneutral.acclo}, \num{rv.cas.nimble.comptwo.doneneutral.acchi}]}} & \num{rv.cas.nimble.comptwo.doneneutral.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.nimble.comptwo.doneneutral.gainlo}, \num{rv.cas.nimble.comptwo.doneneutral.gainhi}]}} & \num{rv.cas.nimble.comptwo.doneneutral.esc} & \num{rv.cas.nimble.comptwo.doneneutral.costfrac} \\
\groupspan{nine}{Escalation to Qwen3.6-27B, likelihood}
\msw{jev}Jev 1.13.0 & \num{e6.jev.comptwoll.doneneutral.accfirst} & \num{e6.jev.comptwoll.doneneutral.accsecond} & \num{rv.cas.jev.comptwoll.doneneutral.acc} & {\scriptsize\cellnote{[\num{rv.cas.jev.comptwoll.doneneutral.acclo}, \num{rv.cas.jev.comptwoll.doneneutral.acchi}]}} & \num{rv.cas.jev.comptwoll.doneneutral.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.jev.comptwoll.doneneutral.gainlo}, \num{rv.cas.jev.comptwoll.doneneutral.gainhi}]}} & \num{rv.cas.jev.comptwoll.doneneutral.esc} & \num{rv.cas.jev.comptwoll.doneneutral.costfrac} \\
\msw{layaen}Laya (English) & \num{e6.layaen.comptwoll.doneneutral.accfirst} & \num{e6.layaen.comptwoll.doneneutral.accsecond} & \num{rv.cas.layaen.comptwoll.doneneutral.acc} & {\scriptsize\cellnote{[\num{rv.cas.layaen.comptwoll.doneneutral.acclo}, \num{rv.cas.layaen.comptwoll.doneneutral.acchi}]}} & \num{rv.cas.layaen.comptwoll.doneneutral.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.layaen.comptwoll.doneneutral.gainlo}, \num{rv.cas.layaen.comptwoll.doneneutral.gainhi}]}} & \num{rv.cas.layaen.comptwoll.doneneutral.esc} & \num{rv.cas.layaen.comptwoll.doneneutral.costfrac} \\
\msw{layaml}Laya (multilingual) & \num{e6.layaml.comptwoll.doneneutral.accfirst} & \num{e6.layaml.comptwoll.doneneutral.accsecond} & \num{rv.cas.layaml.comptwoll.doneneutral.acc} & {\scriptsize\cellnote{[\num{rv.cas.layaml.comptwoll.doneneutral.acclo}, \num{rv.cas.layaml.comptwoll.doneneutral.acchi}]}} & \num{rv.cas.layaml.comptwoll.doneneutral.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.layaml.comptwoll.doneneutral.gainlo}, \num{rv.cas.layaml.comptwoll.doneneutral.gainhi}]}} & \num{rv.cas.layaml.comptwoll.doneneutral.esc} & \num{rv.cas.layaml.comptwoll.doneneutral.costfrac} \\
\msw{kevsmall}Kev-0.8B & \num{e6.kevsmall.comptwoll.doneneutral.accfirst} & \num{e6.kevsmall.comptwoll.doneneutral.accsecond} & \num{rv.cas.kevsmall.comptwoll.doneneutral.acc} & {\scriptsize\cellnote{[\num{rv.cas.kevsmall.comptwoll.doneneutral.acclo}, \num{rv.cas.kevsmall.comptwoll.doneneutral.acchi}]}} & \num{rv.cas.kevsmall.comptwoll.doneneutral.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.kevsmall.comptwoll.doneneutral.gainlo}, \num{rv.cas.kevsmall.comptwoll.doneneutral.gainhi}]}} & \num{rv.cas.kevsmall.comptwoll.doneneutral.esc} & \num{rv.cas.kevsmall.comptwoll.doneneutral.costfrac} \\
\msw{kevlarge}Kev-9B & \num{e6.kevlarge.comptwoll.doneneutral.accfirst} & \num{e6.kevlarge.comptwoll.doneneutral.accsecond} & \num{rv.cas.kevlarge.comptwoll.doneneutral.acc} & {\scriptsize\cellnote{[\num{rv.cas.kevlarge.comptwoll.doneneutral.acclo}, \num{rv.cas.kevlarge.comptwoll.doneneutral.acchi}]}} & \num{rv.cas.kevlarge.comptwoll.doneneutral.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.kevlarge.comptwoll.doneneutral.gainlo}, \num{rv.cas.kevlarge.comptwoll.doneneutral.gainhi}]}} & \num{rv.cas.kevlarge.comptwoll.doneneutral.esc} & \num{rv.cas.kevlarge.comptwoll.doneneutral.costfrac} \\
\msw{decider}decider-2b & \num{e6.decider.comptwoll.doneneutral.accfirst} & \num{e6.decider.comptwoll.doneneutral.accsecond} & \num{rv.cas.decider.comptwoll.doneneutral.acc} & {\scriptsize\cellnote{[\num{rv.cas.decider.comptwoll.doneneutral.acclo}, \num{rv.cas.decider.comptwoll.doneneutral.acchi}]}} & \num{rv.cas.decider.comptwoll.doneneutral.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.decider.comptwoll.doneneutral.gainlo}, \num{rv.cas.decider.comptwoll.doneneutral.gainhi}]}} & \num{rv.cas.decider.comptwoll.doneneutral.esc} & \num{rv.cas.decider.comptwoll.doneneutral.costfrac} \\*
\msw{thisthat}this-that-model-1.0 & \num{e6.thisthat.comptwoll.doneneutral.accfirst} & \num{e6.thisthat.comptwoll.doneneutral.accsecond} & \num{rv.cas.thisthat.comptwoll.doneneutral.acc} & {\scriptsize\cellnote{[\num{rv.cas.thisthat.comptwoll.doneneutral.acclo}, \num{rv.cas.thisthat.comptwoll.doneneutral.acchi}]}} & \num{rv.cas.thisthat.comptwoll.doneneutral.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.thisthat.comptwoll.doneneutral.gainlo}, \num{rv.cas.thisthat.comptwoll.doneneutral.gainhi}]}} & \num{rv.cas.thisthat.comptwoll.doneneutral.esc} & \num{rv.cas.thisthat.comptwoll.doneneutral.costfrac} \\*
\msw{nimble}Nimble-9B & \num{e6.nimble.comptwoll.doneneutral.accfirst} & \num{e6.nimble.comptwoll.doneneutral.accsecond} & \num{rv.cas.nimble.comptwoll.doneneutral.acc} & {\scriptsize\cellnote{[\num{rv.cas.nimble.comptwoll.doneneutral.acclo}, \num{rv.cas.nimble.comptwoll.doneneutral.acchi}]}} & \num{rv.cas.nimble.comptwoll.doneneutral.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.nimble.comptwoll.doneneutral.gainlo}, \num{rv.cas.nimble.comptwoll.doneneutral.gainhi}]}} & \num{rv.cas.nimble.comptwoll.doneneutral.esc} & \num{rv.cas.nimble.comptwoll.doneneutral.costfrac} \\*
\bottomrule
\end{tabular}
\par\vspace{6pt}
\begin{tabular}{P{0.2600}N{0.0850}N{0.0850}N{0.0850}P{0.1300}N{0.0750}P{0.1100}N{0.0850}N{0.0850}}
\toprule
\headrow \hdtop{D2 CLINC-150} & \hdgroup{two}{Single stage} & \hdgroup{four}{Cascade} & \hdgroup{two}{Escalation} \\
\bandrules{2-3,4-7,8-9}
\headrow \hdsub{First stage} & \hdsub{First} & \hdsub{Second} & \hdsub{Accuracy} & \hdsub{} & \hdsub{Gain\mk{}} & \hdsub{} & \hdsub{Esc.} & \hdsub{Cost} \\
\midrule
\tabhead
\groupspan{nine}{Escalation to Qwen3-14B, verbal}
\msw{jev}Jev 1.13.0 & \num{e6.jev.compopen.dtwo.accfirst} & \num{e6.jev.compopen.dtwo.accsecond} & \num{rv.cas.jev.compopen.dtwo.acc} & {\scriptsize\cellnote{[\num{rv.cas.jev.compopen.dtwo.acclo}, \num{rv.cas.jev.compopen.dtwo.acchi}]}} & \num{rv.cas.jev.compopen.dtwo.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.jev.compopen.dtwo.gainlo}, \num{rv.cas.jev.compopen.dtwo.gainhi}]}} & \num{rv.cas.jev.compopen.dtwo.esc} & \num{rv.cas.jev.compopen.dtwo.costfrac} \\
\msw{layaen}Laya (English) & -- & -- & -- &  & --\mk{} &  & -- & -- \\
\msw{layaml}Laya (multilingual) & \num{e6.layaml.compopen.dtwo.accfirst} & \num{e6.layaml.compopen.dtwo.accsecond} & \num{rv.cas.layaml.compopen.dtwo.acc} & {\scriptsize\cellnote{[\num{rv.cas.layaml.compopen.dtwo.acclo}, \num{rv.cas.layaml.compopen.dtwo.acchi}]}} & \num{rv.cas.layaml.compopen.dtwo.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.layaml.compopen.dtwo.gainlo}, \num{rv.cas.layaml.compopen.dtwo.gainhi}]}} & \num{rv.cas.layaml.compopen.dtwo.esc} & \num{rv.cas.layaml.compopen.dtwo.costfrac} \\
\msw{kevsmall}Kev-0.8B & \num{e6.kevsmall.compopen.dtwo.accfirst} & \num{e6.kevsmall.compopen.dtwo.accsecond} & \num{rv.cas.kevsmall.compopen.dtwo.acc} & {\scriptsize\cellnote{[\num{rv.cas.kevsmall.compopen.dtwo.acclo}, \num{rv.cas.kevsmall.compopen.dtwo.acchi}]}} & \num{rv.cas.kevsmall.compopen.dtwo.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.kevsmall.compopen.dtwo.gainlo}, \num{rv.cas.kevsmall.compopen.dtwo.gainhi}]}} & \num{rv.cas.kevsmall.compopen.dtwo.esc} & \num{rv.cas.kevsmall.compopen.dtwo.costfrac} \\
\msw{kevlarge}Kev-9B & \num{e6.kevlarge.compopen.dtwo.accfirst} & \num{e6.kevlarge.compopen.dtwo.accsecond} & \num{rv.cas.kevlarge.compopen.dtwo.acc} & {\scriptsize\cellnote{[\num{rv.cas.kevlarge.compopen.dtwo.acclo}, \num{rv.cas.kevlarge.compopen.dtwo.acchi}]}} & \num{rv.cas.kevlarge.compopen.dtwo.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.kevlarge.compopen.dtwo.gainlo}, \num{rv.cas.kevlarge.compopen.dtwo.gainhi}]}} & \num{rv.cas.kevlarge.compopen.dtwo.esc} & \num{rv.cas.kevlarge.compopen.dtwo.costfrac} \\
\msw{decider}decider-2b & \num{e6.decider.compopen.dtwo.accfirst} & \num{e6.decider.compopen.dtwo.accsecond} & \num{rv.cas.decider.compopen.dtwo.acc} & {\scriptsize\cellnote{[\num{rv.cas.decider.compopen.dtwo.acclo}, \num{rv.cas.decider.compopen.dtwo.acchi}]}} & \num{rv.cas.decider.compopen.dtwo.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.decider.compopen.dtwo.gainlo}, \num{rv.cas.decider.compopen.dtwo.gainhi}]}} & \num{rv.cas.decider.compopen.dtwo.esc} & \num{rv.cas.decider.compopen.dtwo.costfrac} \\
\msw{thisthat}this-that-model-1.0 & \num{e6.thisthat.compopen.dtwo.accfirst} & \num{e6.thisthat.compopen.dtwo.accsecond} & \num{rv.cas.thisthat.compopen.dtwo.acc} & {\scriptsize\cellnote{[\num{rv.cas.thisthat.compopen.dtwo.acclo}, \num{rv.cas.thisthat.compopen.dtwo.acchi}]}} & \num{rv.cas.thisthat.compopen.dtwo.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.thisthat.compopen.dtwo.gainlo}, \num{rv.cas.thisthat.compopen.dtwo.gainhi}]}} & \num{rv.cas.thisthat.compopen.dtwo.esc} & \num{rv.cas.thisthat.compopen.dtwo.costfrac} \\
\msw{nimble}Nimble-9B & \num{e6.nimble.compopen.dtwo.accfirst} & \num{e6.nimble.compopen.dtwo.accsecond} & \num{rv.cas.nimble.compopen.dtwo.acc} & {\scriptsize\cellnote{[\num{rv.cas.nimble.compopen.dtwo.acclo}, \num{rv.cas.nimble.compopen.dtwo.acchi}]}} & \num{rv.cas.nimble.compopen.dtwo.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.nimble.compopen.dtwo.gainlo}, \num{rv.cas.nimble.compopen.dtwo.gainhi}]}} & \num{rv.cas.nimble.compopen.dtwo.esc} & \num{rv.cas.nimble.compopen.dtwo.costfrac} \\
\groupspan{nine}{Escalation to Qwen3.6-27B, verbal}
\msw{jev}Jev 1.13.0 & \num{e6.jev.comptwo.dtwo.accfirst} & \num{e6.jev.comptwo.dtwo.accsecond} & \num{rv.cas.jev.comptwo.dtwo.acc} & {\scriptsize\cellnote{[\num{rv.cas.jev.comptwo.dtwo.acclo}, \num{rv.cas.jev.comptwo.dtwo.acchi}]}} & \num{rv.cas.jev.comptwo.dtwo.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.jev.comptwo.dtwo.gainlo}, \num{rv.cas.jev.comptwo.dtwo.gainhi}]}} & \num{rv.cas.jev.comptwo.dtwo.esc} & \num{rv.cas.jev.comptwo.dtwo.costfrac} \\
\msw{layaen}Laya (English) & -- & -- & -- &  & --\mk{} &  & -- & -- \\
\msw{layaml}Laya (multilingual) & \num{e6.layaml.comptwo.dtwo.accfirst} & \num{e6.layaml.comptwo.dtwo.accsecond} & \num{rv.cas.layaml.comptwo.dtwo.acc} & {\scriptsize\cellnote{[\num{rv.cas.layaml.comptwo.dtwo.acclo}, \num{rv.cas.layaml.comptwo.dtwo.acchi}]}} & \num{rv.cas.layaml.comptwo.dtwo.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.layaml.comptwo.dtwo.gainlo}, \num{rv.cas.layaml.comptwo.dtwo.gainhi}]}} & \num{rv.cas.layaml.comptwo.dtwo.esc} & \num{rv.cas.layaml.comptwo.dtwo.costfrac} \\
\msw{kevsmall}Kev-0.8B & \num{e6.kevsmall.comptwo.dtwo.accfirst} & \num{e6.kevsmall.comptwo.dtwo.accsecond} & \num{rv.cas.kevsmall.comptwo.dtwo.acc} & {\scriptsize\cellnote{[\num{rv.cas.kevsmall.comptwo.dtwo.acclo}, \num{rv.cas.kevsmall.comptwo.dtwo.acchi}]}} & \num{rv.cas.kevsmall.comptwo.dtwo.gain}\mk{\symfull} & {\scriptsize\cellnote{[\num{rv.cas.kevsmall.comptwo.dtwo.gainlo}, \num{rv.cas.kevsmall.comptwo.dtwo.gainhi}]}} & \num{rv.cas.kevsmall.comptwo.dtwo.esc} & \num{rv.cas.kevsmall.comptwo.dtwo.costfrac} \\
\msw{kevlarge}Kev-9B & \num{e6.kevlarge.comptwo.dtwo.accfirst} & \num{e6.kevlarge.comptwo.dtwo.accsecond} & \num{rv.cas.kevlarge.comptwo.dtwo.acc} & {\scriptsize\cellnote{[\num{rv.cas.kevlarge.comptwo.dtwo.acclo}, \num{rv.cas.kevlarge.comptwo.dtwo.acchi}]}} & \num{rv.cas.kevlarge.comptwo.dtwo.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.kevlarge.comptwo.dtwo.gainlo}, \num{rv.cas.kevlarge.comptwo.dtwo.gainhi}]}} & \num{rv.cas.kevlarge.comptwo.dtwo.esc} & \num{rv.cas.kevlarge.comptwo.dtwo.costfrac} \\
\msw{decider}decider-2b & \num{e6.decider.comptwo.dtwo.accfirst} & \num{e6.decider.comptwo.dtwo.accsecond} & \num{rv.cas.decider.comptwo.dtwo.acc} & {\scriptsize\cellnote{[\num{rv.cas.decider.comptwo.dtwo.acclo}, \num{rv.cas.decider.comptwo.dtwo.acchi}]}} & \num{rv.cas.decider.comptwo.dtwo.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.decider.comptwo.dtwo.gainlo}, \num{rv.cas.decider.comptwo.dtwo.gainhi}]}} & \num{rv.cas.decider.comptwo.dtwo.esc} & \num{rv.cas.decider.comptwo.dtwo.costfrac} \\
\msw{thisthat}this-that-model-1.0 & \num{e6.thisthat.comptwo.dtwo.accfirst} & \num{e6.thisthat.comptwo.dtwo.accsecond} & \num{rv.cas.thisthat.comptwo.dtwo.acc} & {\scriptsize\cellnote{[\num{rv.cas.thisthat.comptwo.dtwo.acclo}, \num{rv.cas.thisthat.comptwo.dtwo.acchi}]}} & \num{rv.cas.thisthat.comptwo.dtwo.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.thisthat.comptwo.dtwo.gainlo}, \num{rv.cas.thisthat.comptwo.dtwo.gainhi}]}} & \num{rv.cas.thisthat.comptwo.dtwo.esc} & \num{rv.cas.thisthat.comptwo.dtwo.costfrac} \\
\msw{nimble}Nimble-9B & \num{e6.nimble.comptwo.dtwo.accfirst} & \num{e6.nimble.comptwo.dtwo.accsecond} & \num{rv.cas.nimble.comptwo.dtwo.acc} & {\scriptsize\cellnote{[\num{rv.cas.nimble.comptwo.dtwo.acclo}, \num{rv.cas.nimble.comptwo.dtwo.acchi}]}} & \num{rv.cas.nimble.comptwo.dtwo.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.nimble.comptwo.dtwo.gainlo}, \num{rv.cas.nimble.comptwo.dtwo.gainhi}]}} & \num{rv.cas.nimble.comptwo.dtwo.esc} & \num{rv.cas.nimble.comptwo.dtwo.costfrac} \\
\groupspan{nine}{Escalation to Qwen3.6-27B, likelihood}
\msw{jev}Jev 1.13.0 & \num{e6.jev.comptwoll.dtwo.accfirst} & \num{e6.jev.comptwoll.dtwo.accsecond} & \num{rv.cas.jev.comptwoll.dtwo.acc} & {\scriptsize\cellnote{[\num{rv.cas.jev.comptwoll.dtwo.acclo}, \num{rv.cas.jev.comptwoll.dtwo.acchi}]}} & \num{rv.cas.jev.comptwoll.dtwo.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.jev.comptwoll.dtwo.gainlo}, \num{rv.cas.jev.comptwoll.dtwo.gainhi}]}} & \num{rv.cas.jev.comptwoll.dtwo.esc} & \num{rv.cas.jev.comptwoll.dtwo.costfrac} \\
\msw{layaen}Laya (English) & -- & -- & -- &  & --\mk{} &  & -- & -- \\
\msw{layaml}Laya (multilingual) & \num{e6.layaml.comptwoll.dtwo.accfirst} & \num{e6.layaml.comptwoll.dtwo.accsecond} & \num{rv.cas.layaml.comptwoll.dtwo.acc} & {\scriptsize\cellnote{[\num{rv.cas.layaml.comptwoll.dtwo.acclo}, \num{rv.cas.layaml.comptwoll.dtwo.acchi}]}} & \num{rv.cas.layaml.comptwoll.dtwo.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.layaml.comptwoll.dtwo.gainlo}, \num{rv.cas.layaml.comptwoll.dtwo.gainhi}]}} & \num{rv.cas.layaml.comptwoll.dtwo.esc} & \num{rv.cas.layaml.comptwoll.dtwo.costfrac} \\
\msw{kevsmall}Kev-0.8B & \num{e6.kevsmall.comptwoll.dtwo.accfirst} & \num{e6.kevsmall.comptwoll.dtwo.accsecond} & \num{rv.cas.kevsmall.comptwoll.dtwo.acc} & {\scriptsize\cellnote{[\num{rv.cas.kevsmall.comptwoll.dtwo.acclo}, \num{rv.cas.kevsmall.comptwoll.dtwo.acchi}]}} & \num{rv.cas.kevsmall.comptwoll.dtwo.gain}\mk{\symfull} & {\scriptsize\cellnote{[\num{rv.cas.kevsmall.comptwoll.dtwo.gainlo}, \num{rv.cas.kevsmall.comptwoll.dtwo.gainhi}]}} & \num{rv.cas.kevsmall.comptwoll.dtwo.esc} & \num{rv.cas.kevsmall.comptwoll.dtwo.costfrac} \\
\msw{kevlarge}Kev-9B & \num{e6.kevlarge.comptwoll.dtwo.accfirst} & \num{e6.kevlarge.comptwoll.dtwo.accsecond} & \num{rv.cas.kevlarge.comptwoll.dtwo.acc} & {\scriptsize\cellnote{[\num{rv.cas.kevlarge.comptwoll.dtwo.acclo}, \num{rv.cas.kevlarge.comptwoll.dtwo.acchi}]}} & \num{rv.cas.kevlarge.comptwoll.dtwo.gain}\mk{\symfull} & {\scriptsize\cellnote{[\num{rv.cas.kevlarge.comptwoll.dtwo.gainlo}, \num{rv.cas.kevlarge.comptwoll.dtwo.gainhi}]}} & \num{rv.cas.kevlarge.comptwoll.dtwo.esc} & \num{rv.cas.kevlarge.comptwoll.dtwo.costfrac} \\
\msw{decider}decider-2b & \num{e6.decider.comptwoll.dtwo.accfirst} & \num{e6.decider.comptwoll.dtwo.accsecond} & \num{rv.cas.decider.comptwoll.dtwo.acc} & {\scriptsize\cellnote{[\num{rv.cas.decider.comptwoll.dtwo.acclo}, \num{rv.cas.decider.comptwoll.dtwo.acchi}]}} & \num{rv.cas.decider.comptwoll.dtwo.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.decider.comptwoll.dtwo.gainlo}, \num{rv.cas.decider.comptwoll.dtwo.gainhi}]}} & \num{rv.cas.decider.comptwoll.dtwo.esc} & \num{rv.cas.decider.comptwoll.dtwo.costfrac} \\*
\msw{thisthat}this-that-model-1.0 & \num{e6.thisthat.comptwoll.dtwo.accfirst} & \num{e6.thisthat.comptwoll.dtwo.accsecond} & \num{rv.cas.thisthat.comptwoll.dtwo.acc} & {\scriptsize\cellnote{[\num{rv.cas.thisthat.comptwoll.dtwo.acclo}, \num{rv.cas.thisthat.comptwoll.dtwo.acchi}]}} & \num{rv.cas.thisthat.comptwoll.dtwo.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.thisthat.comptwoll.dtwo.gainlo}, \num{rv.cas.thisthat.comptwoll.dtwo.gainhi}]}} & \num{rv.cas.thisthat.comptwoll.dtwo.esc} & \num{rv.cas.thisthat.comptwoll.dtwo.costfrac} \\*
\msw{nimble}Nimble-9B & \num{e6.nimble.comptwoll.dtwo.accfirst} & \num{e6.nimble.comptwoll.dtwo.accsecond} & \num{rv.cas.nimble.comptwoll.dtwo.acc} & {\scriptsize\cellnote{[\num{rv.cas.nimble.comptwoll.dtwo.acclo}, \num{rv.cas.nimble.comptwoll.dtwo.acchi}]}} & \num{rv.cas.nimble.comptwoll.dtwo.gain}\mk{} & {\scriptsize\cellnote{[\num{rv.cas.nimble.comptwoll.dtwo.gainlo}, \num{rv.cas.nimble.comptwoll.dtwo.gainhi}]}} & \num{rv.cas.nimble.comptwoll.dtwo.esc} & \num{rv.cas.nimble.comptwoll.dtwo.costfrac} \\*
\bottomrule
\end{tabular}
\tablenote{First and Second are the accuracies of each stage alone, Accuracy is the cascade accuracy with thresholds chosen on data disjoint from the scored items, and Gain is its difference from the better single stage in points. Esc.\ is the escalated share and Cost the cost fraction from each decision's own cost, where the escalation unit on D1 is the decision, a request's cost is shared among its decisions and a comparator is charged per question. Brackets hold cluster bootstrap intervals at \num{p.boot.level} percent whose \num{p.boot.refitreps} replicates refit the thresholds, unadjusted for the number of cascades. A dash marks a pair without results, because Laya (English) refused the full intent list, and \symfull\ marks a gain whose interval excludes zero.}

